The Analysis and the Performance of the Parallel-Partial Reset Control System

Reset controllers have demonstrated their effectiveness in enhancing performance in precision motion systems. To further exploiting the potential of reset controllers, this study introduces a parallel-partial reset control structure. Frequency response analysis is effective for the design and fine-tuning of controllers in industries. However, conducting frequency response analysis for reset control systems poses challenges due to their nonlinearities. We develop frequency response analysis methods for both the open-loop and closed-loop parallel-partial reset systems. Simulation results validate the accuracy of the analysis methods, showcasing precision enhancements exceeding 100% compared to the traditional describing function method. Furthermore, we design a parallel-partial reset controller within the Proportional-Integral-Derivative (PID) control structure for a mass-spring-damper system. The frequency response analysis of the designed system indicates that, while maintaining the same bandwidth and phase margin of the first-order harmonics, the new system exhibits lower magnitudes of higher-order harmonics, compared to the traditional reset system. Moreover, simulation results demonstrate that the new system achieves lower overshoot and quicker settling time compared to both the traditional reset and linear systems.

==> 0Methodology0.tex <==
\section{Frequency-domain Method to determine two-reset and multiple-reset regions}
\label{sec:methodology}
This section first proposes the piece-wise model for a general SSISO RCS. Then, based on this model, a frequency-domain-based method to determine the two-reset and multiple-reset regions in a general RCS is developed.
\subsection{Piece-wise Representatives of General RCSs}%
\label{subsec: Piece-wise function}
\begin{lem}
	Neglecting the initial transient response of the system, the first reset instant $t_1 \in t_R$ of a RCS with sinusoidal reference input signal $r(t) = A\sin (\omega t)$ is given by
	\begin{equation}
		\label{eq: t1}
		t_{1} = \frac{\pi-\angle\mathcal{S}_{bl}(\omega)}{\omega}.
	\end{equation}
\end{lem}
\begin{proof}
	The first reset action occurs when the base-linear error signal $e_{bl}(t)$ crosses zero, which is given by
	\begin{equation}
		\label{eq: e_bl(t)}
		e_{bl}(t) = A|\mathcal{S}_{bl}|(\omega)\sin(\omega t + \angle\mathcal{S}_{bl}(\omega)) = 0,
	\end{equation}
	then the first solution of $e_{bl}(t_1) = 0$ is the first reset instant $t_1$ of the $\mathcal{RCS}$ as shown in \eqref{eq: t1}.
\end{proof}
\begin{thm}
\label{thm: piece-wise function}
The outputs of a general SISO RCS under a sinusoidal reference input signal $r(t) = A\sin(\omega t)$ are piece-wise functions separated by reset instants $t_i \in t_R$. During two arbitrary reset instants $(t_i, t_{i+1})$, the control input signal $u_{i+1}(t)$, output signal $y_{i+1}(t)$, and error signal $e_{i+1}(t)$ are given as below.
\begin{equation}
\label{eq: piecewise reset outputs}
\begin{aligned}
    u_{i+1}(t-t_i) &= u_{i}(t-t_{i-1})-(1-\gamma)u_{i}(t_i)\cdot h_s(t-t_i),\\
    y_{i+1}(t-t_i) &= y_{i}(t-t_{i-1})-(1-\gamma)u_{i}(t_i)\cdot h_{ps}(t-t_i),\\
    e_{i+1}(t-t_i) &= e_{i}(t-t_{i-1})+(1-\gamma)u_{i}(t_i)\cdot h_{ps}(t-t_i),
\end{aligned}
\end{equation}
where
$h_s(t)$ and $h_{ps}(t)$ are step responses of the transfer functions $\mathcal{R}_{\delta}(\omega)\mathcal{S}_{bl}(\omega)$ and $\mathcal{R}_{\delta}(\omega)\mathcal{P}(\omega)\mathcal{S}_{bl}(\omega)$ given by
\begin{equation}
\label{eq: R_delta, hps, hs}
    \begin{aligned}
         h_s(t) &= \mathscr{F}^{-1}[H(\omega)\cdot \mathcal{R}_{\delta}(\omega)\mathcal{S}_{bl}(\omega)],\\
         h_{ps}(t) &= \mathscr{F}^{-1}[H(\omega)\cdot \mathcal{R}_{\delta}(\omega)\mathcal{P}(\omega)\mathcal{S}_{bl}(\omega)],\\
         \mathcal{R}_{\delta}(\omega) &= C_R(j\omega I-A_R)^{-1}j\omega I\\
         H(\omega) &= \mathscr{F}[h(t)] = \frac{1}{j\omega},\\
         h(t)&:={\begin{cases}1,&t>0\\0,&t\leq 0\end{cases}}.
    \end{aligned}
\end{equation}
\end{thm}
\begin{proof}
    At a reset instant $t_i$ in $t_R$ where $i \in \mathbb{N}$, the state $x(t_i)$ of the system resets to its proportional value of $\gamma x(t_i)$. This reset is equivalent to introducing a step signal $(\gamma-1)u_{i}(t_i)h(t-t_i)$, which is considered a disturbance to $x(t)$ during the time interval $(t_i, t_{i+1})$, as illustrated in Figure \ref{fig1:RCS_piece}(b).
    \begin{figure}[htp]
	%	\missingfigure{RCsystem}
	\centerline{\includegraphics[width=\columnwidth]{figs/Block diagrams of reset controller.pdf}}
	\caption{The block diagrams of the RC ($\mathcal{C}$ in red) during $(t_i, \ t_{i+1})$, where (a) is based on the \eqref{eq: State-Space eq of RC} and (b) corresponds to \eqref{eq: piecewise reset outputs}. $e_i(t)$, $x_i(t)$, $x_{bl}(t)$, and $u_i(t)$ are the input, state, base-linear state, and output signals of the RC, respectively. The blue lines are reset-related signals, and the grey box represents the base-linear controller $\mathcal{C}_{bl}$.}
	\label{fig1:RCS_piece}
\end{figure}

Then, the control input signal $u_{i+1}(t)$ during $(t_i, t_{i+1})$ is given by
\begin{equation}
    u_{i+1}(t-t_i) = u_{i}(t-t_{i-1})-(1-\gamma)u_{i}(t_i)\cdot h_s(t-t_i).
\end{equation}
Similarly, $y_{i+1}(t)$ and $e_{i+1}(t)$ in  \eqref{eq: piecewise reset outputs} can be derived.
 \end{proof} 
%  Examples comparing the $y(t)$ and $e(t)$ using Simulink and applying \eqref{eq: piecewise reset outputs} of three different RCSs in closed-loop: a) the first order $\mathcal{RC}$ ($CI$), b) the second order $\mathcal{RC}$ ($SORE$), and c) a $\mathcal{RCS}$ ($CI \text{ and a first-order plant} \frac{1}{s+1}$) are shown in Fig. \ref{fig:ex3}.
%  \begin{figure}[h]
%      \centering
%      \begin{subfigure}[b]{0.155\textwidth}
%          \centerline{\includegraphics[width=\columnwidth]{figs/multiple_reset_ci.eps}}
% 	    \caption{CI.}
% 	    \label{fig: ex_cl_in_closed_loop}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.155\textwidth}
%          \centerline{\includegraphics[width=\columnwidth]{figs/multiple_reset_sore.eps}}
% 	    \caption{SORE.}
% 	    \label{fig: SORE_in_closed_loop}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.155\textwidth}
%          \centerline{\includegraphics[width=\columnwidth]{figs/com_y_e.eps}}
% 	    \caption{CI + Plant.}
% 	    \label{fig: CI + Plant _closed_loop}
%      \end{subfigure}
%     \caption{Multiple resets example of CI in Closed-loop.}
%     \label{fig:ex3}
%     \end{figure}
\subsection{Frequency-domain Condition for Multiple-reset Cases}
This subsection develops the frequency-domain method to determine the regions of multiple resets and two resets per period in RCSs.
% When $e_{bl}(t)$ has no more than two zero-crossing points during $(0, \pi/\omega)$, then
\begin{thm}
\label{thm: Delta}
    In a SISO closed-loop RCS with sinusoidal reference input signal $r(t) = A\sin (\omega t)$, the occurrence of multiple-reset is characterised by the first solution of $\Delta(\omega) > 0$, where
    \begin{enumerate}
        \item when $\mathcal{P}$ is a first order plant,
        \begin{equation}
        \label{eq: 1stplant}
            \begin{aligned}
                \Delta(\omega) &= -\omega|\mathcal{S}_{bl}(\omega)| - k_1(1-\gamma)|\mathcal{CS}_{bl}(\omega)|\sin (\angle \mathcal{C}_{bl}(\omega)),\\
                k_1 &= \lim\limits_{s\to \infty}  s\mathcal{R}_{\delta}(s)\mathcal{P}(s)\mathcal{S}_{bl}(s).
            \end{aligned}
        \end{equation}
        \item When $\mathcal{P}$ is a second order plant,
        \begin{equation}
         \label{eq:2ndplant}
            \begin{aligned}
                \Delta(\omega) = &-\omega|\mathcal{S}_{bl}(\omega)| \cos(\omega t_p/3)- k_2t_p(1-\gamma)\cdot\\& |\mathcal{CS}_{bl}(\omega)|\sin (\angle \mathcal{C}_{bl}(\omega))/3,\\
                k_2 = &\lim\limits_{s\to \infty}  s^2\mathcal{R}_{\delta}(s)\mathcal{P}(s)\mathcal{S}_{bl}(s).
            \end{aligned}
        \end{equation}
    \end{enumerate}
% \begin{equation}
%     k = \lim _ {s\to \infty} s\mathcal{R}_{\delta}(s)\mathcal{P}(s)\mathcal{S}_{bl}(s).
% \end{equation}
% $\Lambda(\omega)$ is given by
% \begin{equation}
% \resizebox{.97\hsize}{!}{$
% \begin{aligned}
%  \Lambda(\omega) &= -\omega|\angle \mathcal{S}_{bl}(\omega)|-(1-\gamma)|\mathcal{CS}_{bl}|(\omega)\cdot \sin(\mathcal{L}_{bl}(\omega))\cdot k,\\
%     % \Lambda(\omega) &= \cos(\angle\mathcal{L}_{bl}(\omega))(|\mathcal{T}_{bl}|(\omega)-1)-(1-\gamma)|\mathcal{CS}_{bl}|(\omega)\cdot \sin(\mathcal{L}_{bl}(\omega))\cdot k,\\
%     k &= \lim _ {s\to \infty} s\mathcal{R}_{\delta}(s)\mathcal{P}(s)\mathcal{S}_{bl}(s).
% \end{aligned}$}
% \end{equation}
$t_p$ is defined as the peak time of $h'_{ps}(t)$ that can be easily obtained by the step response of the BLS; $\mathcal{C}_{bl}(\omega)$ is the transfer function of the base-linear controller; $\mathcal{S}_{bl}(\omega)$, $\mathcal{CS}_{bl}(\omega)$,  $\mathcal{P}(s)\mathcal{S}_{bl}(s)$, and $\mathcal{R}_{\delta}(s)$ can be found in \eqref{eq: L_bl}, \eqref{eq: gang of four} and \eqref{eq: R_delta, hps, hs} respectively.
\end{thm}
\begin{proof}
In a general SISO closed-loop RCS with sinusoidal reference input signal $r(t) = A\sin (\omega t)$, multiple-reset occurs when there are more than two resets in one period. Reset instants $t_i \in t_R$ satisfy the condition $e(t_i) = r(t_i) - y(t_i) = 0$, where the first reset instant $t_1$ is given by \eqref{eq: t1}. Thus, the condition for multiple-reset is equivalent to having at least one additional zero in $e(t)$ during $t \in (t_1, \pi/\omega)$. More specifically, the boundary condition for multiple-reset is satisfied when $e_2(t-t_1)=0$.\\
% $e_2(t-t_1) = r(t) - y_2(t-t_1) =0$.
% Then the condition of multiple-reset can be transferred into that there is at least one more zero of $e(t)$ during $t \in (t_1, \pi/\omega)$. 
% As demonstrated in Theorem \ref{thm: piece-wise function}, $e(t)$ is a piece-wise function.
% \begin{equation}
%         e_2(t-t_1) = e_{bl}(t)+(1-\gamma)u_{bl}(t_1)\cdot h_{ps}(t-t_1) = 0.
% \end{equation}
% The nonlinear element of $e_2(t-t_1)$ is a step response of $\mathcal{R}_{\delta}(s)\mathcal{P}(s)\mathcal{S}_{bl}(s)$, which is given by
% \begin{equation}
%     e_{2nl}(t-t_1) = (1-\gamma)u_{bl}(t_1)\cdot h_{ps}(t-t_1).
% \end{equation}
% Let $t^* = t-t_1$, then we have
% \begin{equation}
%     e_{2nl}(t^*) = (1-\gamma)u_{bl}(t_1)\cdot h_{ps}(t^*).
% \end{equation}
% The infinite output of $e_{2nl}(t^*)$ is given by
% \begin{equation}
%     \lim_{t^*\to \infty}e_{2nl}(t^*) = \lim_{s\to 0}(1-\gamma)u_{bl}(t_1)\cdot \mathcal{R}_{\delta}(s)\mathcal{P}(s)\mathcal{S}_{bl}(s)=0,
% \end{equation}
% which means that the nonlinear step response will die out with time, thus we have
% \begin{equation}
%     \lim_{t^*\to \infty}e_2(t-t_1) = e_{bl}(t),
% \end{equation}
% that shows the $e_2(t-t_1)$ tends to $e_{bl}(t)$.
Based on \eqref{eq: piecewise reset outputs}, $e_2(t-t_1)$ is given by 
\begin{equation}
        e_2(t-t_1) = e_{bl}(t)+(1-\gamma)u_{1}(t_1)\cdot h_{ps}(t-t_1),
\end{equation}
where $u_{1}(t_1) = u_{bl}(t_1)$.\\
% The nonlinear element of $y_2(t-t_1)$ is a step response of $\mathcal{R}_{\delta}(s)\mathcal{P}(s)\mathcal{S}_{bl}(s)$, which is given by
Let
\begin{equation}
    e_{2nl}(t-t_1) = (1-\gamma)u_{bl}(t_1)\cdot h_{ps}(t-t_1),
\end{equation}
then $e_2(t-t_1)$ is given by
\begin{equation}
    e_2(t-t_1) = e_{1}(t) + e_{2nl}(t-t_1),
\end{equation}
with $e_1(t) = e_{bl}(t)$.\\
Define $t^* = t-t_1$, then we have
\begin{equation}
\label{eq: e2nl}
    e_{2nl}(t^*) = (1-\gamma)u_{bl}(t_1)\cdot h_{ps}(t^*).
\end{equation}
Suppose that $E_{2nl}(s)$ is the Laplace transform of $e_{2nl}(t^*)$, which is given by
\begin{equation}
    E_{2nl}(s) = (1-\gamma)u_{bl}(t_1)H(s)\mathcal{R}_{\delta}(s)\mathcal{P}(s)\mathcal{S}_{bl}(s),
\end{equation}
then the steady-state value of $E_{2nl}(t^*)$ is given by
\begin{equation}
\begin{aligned}
    \lim_{t^*\to \infty} e_{2nl}(t^*) &= \lim_{s\to 0} sE_{2nl}(s) = 0,
    % & = \lim\limits_{s\to 0}-s(1-\gamma)u_{bl}(t_1)\cdot H(s)\mathcal{R}_{\delta}(s)\mathcal{P}(s)\mathcal{S}_{bl}(s)=0,
\end{aligned}
\end{equation}
which means that $e_{2nl}(t^*)$ will die out with time, thus we have
\begin{equation}
\begin{aligned}
    %  \lim_{t^*\to \infty}y_2(t^*) &= y_{bl}(t),\\
     \lim_{t^*\to \infty}e_2(t^*) &= e_{bl}(t),
\end{aligned}
\end{equation}
that demonstrates $e_2(t^*)$ tends to $e_{bl}(t)$ with time.

% When $0<\angle \mathcal{S}_{bl}(\omega) < \frac{\pi}{2}$,\\
Accordingly, to make sure that $e_2(t^*) = 0$ has solutions when $t>t_1$, we need to guarantee that
\begin{equation}
\label{eq: condi}
    e'_2(t_1)\cdot e'_{bl}(t_1) <0,
\end{equation}
where $e'_{bl}(t_1)$ is the derivative of $e_{bl}(t)$ at $t_1$ given by
% \begin{equation}
%     r'(t) = A\cdot \omega \cos(\omega t).
% \end{equation}
%  is given by
\begin{equation}
    e'_{bl}(t_1) = -A|\mathcal{S}_{bl}|(\omega)\omega < 0.
\end{equation}
Now, we need to guarantee $e'_2(t_1)>0$ to satisfy \eqref{eq: condi}.

$e'_{2nl}(t_1)$ is given by 
% \begin{equation}
% \begin{aligned}
%     \lim_{t^*\to 0} y_{2nl}(t^*) &= \lim_{s\to \infty} sY_{2nl}(s)\\
%     &= -(1-\gamma)u_{bl}(t_1) \lim_{s\to \infty} \mathcal{R}_{\delta}(s)\mathcal{P}(s)\mathcal{S}_{bl}(s).
% \end{aligned}
% \end{equation}
% The derivative of $y_{2nl}'(t^*)$ at $t^* = 0$ is given by
\begin{equation}
\label{eq: e'2nl}
\begin{aligned}
    e'_{2nl}(t_1) &= \lim_{t^*\to 0} e_{2nl}'(t^*) = \lim_{s\to \infty} s^2E_{2nl}(s)\\
    &= (1-\gamma)u_{bl}(t_1) \lim_{s\to \infty} s\mathcal{R}_{\delta}(s)\mathcal{P}(s)\mathcal{S}_{bl}(s)
\end{aligned}
\end{equation}
% For the first order plant, $e'_{2nl}(t_1)$ can be derived by \eqref{eq: e'2nl}. 
Thus, $e_{2}'(t_1)$ in a first order plant is given by
\begin{equation}
    \label{eq: e2'}
    \begin{aligned}
        e_{2}'(t_1) &= e_{bl}'(t_1) + e_{2nl}'(t_1)\\
        &= -A|\mathcal{S}_{bl}|(\omega)\omega + (1-\gamma)u_{bl}(t_1) \lim_{s\to \infty}s \mathcal{R}_{\delta}(s)\mathcal{P}(s)\mathcal{S}_{bl}(s)\\
        &= -A|\mathcal{S}_{bl}|(\omega)\omega - Ak_1|\mathcal{CS}_{bl}|(\omega)\sin(\angle\mathcal{C}_{bl}(\omega)) ,
    \end{aligned}
\end{equation}
where $k_1$ is defined as
\begin{equation}
    k_1 = \lim_{s\to \infty} s\mathcal{R}_{\delta}(s)\mathcal{P}(s)\mathcal{S}_{bl}(s).
\end{equation}
In a RCS with first order plant, $\Delta(\omega)$ is defined as
\begin{equation}
\label{eq: V1}
% \resizebox{.97\hsize}{!}{$
\begin{aligned}
\Delta(\omega) &= \frac{e_{2}'(t_1)}{A}.
\end{aligned}
% $}
\end{equation}
Then, equation \eqref{eq: 1stplant} for the RCS with first order plant is derived by substituting \eqref{eq: e2'} and \eqref{eq: V1} to \eqref{eq: condi}.

In the context of a second-order plant, utilising \eqref{eq: e'2nl}, we have $e_{2nl}'(t_1) = 0$. Consequently, based on \eqref{eq: e2'}, it follows that $e_{2}'(t_1) = e_{2bl}'(t_1)$. Therefore, the condition for multiple-reset specified in \eqref{eq: condi} for the first-order plant is not applicable to the second-order plant case. The ensuing content outlines the procedure for determining the multiple-reset condition for this scenario.

$e''_{bl}(t)$ is given by
\begin{equation}
    e''_{bl}(t) = -A \omega ^2 |\mathcal{S}_{bl}|(\omega)\sin(\omega t +\angle\mathcal{S}_{bl}(\omega)).
\end{equation}
Based on $t_1$ given in \eqref{eq: t1}, we can obtain that $e''_{bl}(t) > 0$ when $t \in (t_1,\pi/\omega)$.

$t_p$ denotes the time of peak value of $e'_{2nl}(t)$ within the interval $(t_1, \pi/\omega)$. It is equivalent to the peak time of $h'_{ps}(t)$, which can be readily determined using the BLS. Consequently, $e''_{2nl}(t)>0$ during $(t_1,\ t_1+t_p)$, and since $e'_2(t) = e'_{bl}(t)+e'_{2nl}(t)$, it follows that $e''_2(t) = e''_{bl}(t)+e''_{2nl}(t) >0$ during $(t_1,\ t_1+t_p)$. Hence, $e''_2(t)$ is monotonically increasing within this interval. 

By selecting a short interval of $t_p/3$, we obtain:
\begin{equation}
    e'_2(t_1+t_p/3) = e'_{bl}(t_1+t_p/3)+e'_{2nl}(t_1+t_p/3) > e'_2(t_1).
\end{equation}

Similarly to \eqref{eq: condi}, the multiple-reset region in the system with second order plant should meet the following condition:
\begin{equation}
\label{eq: condi2}
    e'_{2}(t_1+t_p/3) \cdot e'_{bl}(t_1+t_p/3) < 0.
\end{equation}
Since $t_1+t_p/3 \in (t_1,\ \pi/\omega)$, we have
\begin{equation}
    e_{bl}'(t_1+t_p/3) = -A\omega|\mathcal{S}_{bl}(\omega)| \cos(\omega t_p/3) < 0.
\end{equation}
Then, we need to guarantee $e'_2(t_1+t_p/3)>0$ to satisfy \eqref{eq: condi2}.

$e''_{2nl}(t_1)$ is given by
\begin{equation}
\begin{aligned}
    e''_{2nl}(t_1) &= (1-\gamma)u_{bl}(t_1) \lim_{s\to \infty} s^2\mathcal{R}_{\delta}(s)\mathcal{P}(s)\mathcal{S}_{bl}(s).
\end{aligned}
\end{equation}
As $t_p/3$ is a transient time which is short enough that $e'_{2nl}(t_1+t_p/3)$ can be approximately given by
\begin{equation}
    e'_{2nl}(t_1+t_p/3) \approx e''_{2nl}(t_1) \cdot t_p/3.
\end{equation}\\
% From \eqref{eq: e2nl}, we can easily know that $e_{2nl}(t)$ is a step response with maximum value at peak time defined by $t_p$. During $(t_1, \pi/\omega)$, $e'_{bl}(t) < 0$. Since $e_2(t) = e_{bl}(t)+e_{2nl}(t)$, the maximum value of $e_2(t)$ is located at $t_p$.
% because of the time-delay in the transient response as shown in Fig. \ref{fig1:step_response}, we have $e'_{2nl}(t_1) = 0$. 
% \begin{figure}[htp]
% 	%	\missingfigure{RCsystem}
% 	\centerline{\includegraphics[width=0.7\columnwidth]{figs/step_response.pdf}}
% 	\caption{Step responses of control systems with four second order plants.}
% 	\label{fig1:step_response}
% \end{figure}
Thus, $e_{2}'(t_1+t_p/3)$ is given by
\begin{equation}
    \label{eq: e2'_2ndplant}
    \begin{aligned}
        e_{2}'(t_1+t_p/3)= & e_{bl}'(t_1+t_p/3) + e_{2nl}'(t_1+t_p/3)\\
        =& A|\mathcal{S}_{bl}(\omega)|\cos[\omega (t_1+t_p/3) + \angle \mathcal{S}_{bl}(\omega)] +\\ 
        &(1-\gamma)u_{bl}(t_1) \lim_{s\to \infty}s^2 \mathcal{R}_{\delta}(s)\mathcal{P}(s)\mathcal{S}_{bl}(s)\cdot t_p/3.
    \end{aligned}
\end{equation}
Substitute $t_1$ in \eqref{eq: t1} and $u_{bl}(t)$ based on \eqref{eq: base-linear signals} into \eqref{eq: e2'_2ndplant}, we have
\begin{equation}
\label{eq: e2'_2ndplant2}
\begin{aligned}
     e_{2}'(t_1+t_p/3) = &-A\omega|\mathcal{S}_{bl}(\omega)| \cos(\omega t_p/3)- Ak_2(1-\gamma)\cdot\\
     &|\mathcal{CS}_{bl}(\omega)|\sin (\angle \mathcal{C}_{bl}(\omega))\cdot t_p/3,
\end{aligned}
\end{equation}
where
\begin{equation}
     k_2 = \lim_{s\to \infty} s^2\mathcal{R}_{\delta}(s)\mathcal{P}(s)\mathcal{S}_{bl}(s).
\end{equation}
In a RCS with second order plant, $\Delta(\omega)$ is defined as
\begin{equation}
\label{eq: Delta2}
% \resizebox{.97\hsize}{!}{$
\begin{aligned}
\Delta(\omega) &= \frac{e_{2}'(t_1+t_p/3)}{A},
\end{aligned}
% $}
\end{equation}
Therefore, equation \eqref{eq:2ndplant} for the RCS with second order plant is derived by substituting \eqref{eq: e2'_2ndplant2} and \eqref{eq: Delta2} to \eqref{eq: condi2}. Here we conclude the proof.
\end{proof}
% When $t \in (t_1, \pi/\omega)$, it can be derived as
% \begin{equation}
%     \begin{cases}
%         e_{bl}(t) <0, \ &\text{when }  e'_{bl}(t_1) <0\\
%         e_{bl}(t) >0, \ &\text{when }  e'_{bl}(t_1) >0
%     \end{cases}
% \end{equation}
% $e_2'(t)$ is given by
% \begin{equation}
%     e_2'(t) = e_{bl}'(t)+e_{2nl}'(t^*).
% \end{equation}
% During the start of $(t_1, \frac{\pi}{\omega})$, there are 3 stages:\\
% Stage 1 $(t_1,t_p)$:
% \begin{equation}
%     \begin{aligned}
%         e_{bl}(t)  < 0\  \& \ e_{bl}'(t) <0;\\
%         e_{2nl}(t) > 0\  \& \ e_{2nl}'(t) > 0.
%     \end{aligned}
% \end{equation}
% Stage 2 $(t_p, t_1+\pi/(2\omega))$:
% \begin{equation}
%     \begin{aligned}
%         e_{bl}(t)  < 0\  \& \ e_{bl}'(t) < 0;\\
%         e_{2nl}(t) > 0\  \& \ e_{2nl}'(t) > 0.
%     \end{aligned}
% \end{equation}
% Stage 3 $(t_1+\pi/(2\omega), \pi/\omega)$:
% \begin{equation}
%     \begin{aligned}
%         e_{bl}(t)  < 0\  \& \ e_{bl}'(t) > 0;\\
%         e_{2nl}(t) > 0\  \& \ e_{2nl}'(t) > 0.
%     \end{aligned}
% \end{equation}
% To make sure there are multiple-reset exist, at beginning the following condition need to be met. 
% \begin{equation}
%     e_{bl}(t)\cdot e_{2nl}(t^*)<0.
% \end{equation}
% Then $e_2'(t) = e_{bl}'(t)+e_{2nl}'(t^*)$ first $<0$ and then $>0$. $e_2'(t) = 0$ has solution between $(t_1+\pi/(2\omega), \pi/\omega)$. Thus, $e_2(t)$ first decrease and then increase. $e_2(t)$ finally tends to and has phase delay with $e_{bl}(t)$ because the opposite direction between $e_{bl}(t)$ and $e_{2nl}(t^*)$. Thus, the maximum value of $e_2(t)$ in $(t_1,\frac{\pi}{\omega})$ is $e_2'(t_1)$. 
% Think it later.
% Because of transient response the at the precise first reset instant $t_1$ (\textcolor{blue}{What about get the precise $t_1$? Then the certification tool will not have error.})
% \begin{equation}
%     e''_{bl}(t_1)  >0,
% \end{equation}
% which means the increase speed of $e_{bl}$ will increase, while the increase speed of $e_{2nl}(t^*)$ will decrease (from the rise time). The $e_{2nl}(t^*)$ will die out quickly, thus to make sure that $e_2(t-t_1)=0$ has solution when $t \in (t_1, \pi/\omega)$, we have
%     \begin{equation}
%     \begin{cases}
%     \label{eq: condi}
%       e_{2}'(t_1) > 0,  \ &\text{when }  e'_{bl}(t_1) < 0\\
%       e_{2}'(t_1) < 0,  \ &\text{when } e'_{bl}(t_1) > 0
%     \end{cases}
%     \end{equation}
% \textit{\textcolor{blue}{Explain it analytically?}}\\
\begin{rem}
\label{rem: single_controller}
In a SISO closed-loop RCS with sinusoidal reference input $r(t) = A\sin(\omega t)$ and $\mathcal{P} = 1$, certain frequencies which satisfy $\angle \mathcal{S}_{bl}(\omega) \approx m\pi/\omega$ for $m\in \mathbb{N}$ indicate that $e_{bl}(t)$ and $r(t)$ approximately have the same zero-crossing points. In this case, multiple resets per period will not occur. Hence, for $\mathcal{P}=1$, multiple resets occur if both $\angle \mathcal{S}_{bl}(\omega) \neq m\pi/\omega$ with $m\in \mathbb{N}$ and $\Delta(\omega)>0$ based on \eqref{eq: 1stplant} are satisfied.
\end{rem}
\begin{rem}
\label{rem: ebl_mrcs}
If a SISO closed-loop RCS with sinusoidal reference signal $r(t) = A\sin(\omega t)$ exhibits more than two zero-crossing points in $e_{bl}(t)$ during the initial transient period, it indicates poor design and multiple-reset will occur. 
\end{rem}
The case of inputting the noise signal $n(t)$ to a SSISO RCS is equivalent to inputting the reference input signal $-r(t)$. The following Remark shows the multiple-reset condition for this case.
\begin{rem}
\label{rem: Lambda}
    For a SSISO RCS with the noise input signal $n(t) = N\sin (\omega t)$, multiple-reset occurs at the first solution of $\Delta(\omega) < 0$, where $\Delta(\omega)$ is given in Theorem \ref{thm: Delta}.
\end{rem}    
Similar to the derivation process of Theorem \ref{thm: Delta}, the subsequent remarks provide the multiple-reset conditions for the SSISO RCS with the process disturbance $d(t)$.
\begin{rem}
\label{rem: Lambda}
    For a SSISO RCS with the process disturbance input signal $d(t) = D\sin (\omega t)$, multiple-reset occurs at the first solution of $\Lambda(\omega) > 0$, where
    \begin{enumerate}
        \item when $\mathcal{P}$ is a first order plant,
        \begin{equation}
        \label{eq: 1stplant_d}
            \begin{aligned}
                \Lambda(\omega) = \ &\omega|\mathcal{P}(\omega)\mathcal{S}_{bl}(\omega)| - k_1(1-\gamma)|\mathcal{T}_{bl}(\omega)|\cdot\\&\sin (\angle (\mathcal{P}(\omega)\mathcal{S}_{bl}(\omega)) - \angle \mathcal{T}_{bl}(\omega)).
            \end{aligned}
        \end{equation}
        \item When $\mathcal{P}$ is a second order plant,
        \begin{equation}
         \label{eq:2ndplant}
            \begin{aligned}
                \Lambda(\omega) = \ &\omega|\mathcal{P}(\omega)\mathcal{S}_{bl}(\omega)|\cos(\omega t_p) - k_2t_p(1-\gamma)\cdot\\&|\mathcal{T}_{bl}(\omega)|\sin (\angle (\mathcal{P}(\omega)\mathcal{S}_{bl}(\omega)) - \angle \mathcal{T}_{bl}(\omega))/3.
            \end{aligned}
        \end{equation}
    \end{enumerate}
    % \begin{equation}
    % \label{eq: Lamdba(w)}
    % \resizebox{.97\hsize}{!}{$
    % \Lambda(\omega) = |\mathcal{PS}_{bl}|(\omega)\omega - k(1-\gamma)|\mathcal{T}_{bl}|(\omega)\sin (\angle \mathcal{PS}_{bl}(\omega) - \angle \mathcal{T}_{bl}(\omega)) < 0,$}
    % \end{equation}
% where $k$ is given by
% \begin{equation}
%     k = \lim _ {s\to \infty} s\mathcal{R}_{\delta}(s)\mathcal{P}(s)\mathcal{S}_{bl}(s).
% \end{equation}
\end{rem}




==> 0Results.tex <==
\section{Illustrative Examples}
\label{sec: result}
% Figure \ref{fig:RCS_2p} shows the block diagram of a RCS in closed-loop. This RCS is applied to validate the effectiveness of the multiple-reset condition in Theorem \ref{thm: Delta}. Figure \ref{fig:DL} shows $\Delta(\omega)$ and $\Lambda(\omega)$ of this RCS at different frequencies calculated by \eqref{eq: V(w)} and \eqref{eq: Lamdba(w)}. $\Delta'(\omega)= e'_2(\Bar{t}_1)$ will be discussed in the next section, where $\Bar{t}_1$ is the first reset instant calculated by considering the transient response.
We selected three SSISO RCSs with sinusoidal reference input signal $r(t)$, disturbance signal $d(t)$, and noise signal $n(t)$ by simulation to assess the efficacy of the multiple-reset conditions stated in Theorem \ref{thm: Delta}, Remark \ref{rem: -Delta}, and Remark \ref{rem: Lambda}.

Table \ref{tb:v(w)} shows the base-linear transfer functions of the RCS cases, where $k_{p} =24$, $\omega_r = 2$ rad/s, $\omega_p = 150$ rad/s, $\zeta = 2$, and $\omega_i = 5$ rad/s. $\gamma$ is the reset value.
\begin{table}[htp]
\caption{Reset control system cases}
\label{tb:v(w)}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccc}
Cases &  $\mathcal{C}_{bl}(s)$ & $\mathcal{P}(s)$ & $\gamma$ \\ \hline 
\\[-1em]
case 1 & $\frac{1}{s}$ & $\frac{1}{s+2}$ & 0  \\ 
\\[-0.5em]
case 2 & $k_{p}\cdot\frac{\omega_r}{s+\omega_r}$  & $\frac{\omega_p^2}{s^2 + 2\zeta\omega_p s + \omega_p^2}$ & 0 \\  
\\[-0.5em]
case 3 & $k_{p}\cdot\frac{\omega_r}{s+\omega_r}$  & $\frac{\omega_p^2}{s^2 + 2\zeta\omega_p s + \omega_p^2}$ & -0.2 \\ 
\\[-0.5em]
case 4 & $k_{p}\cdot\frac{\omega_r}{s+\omega_r}$  & $\frac{\omega_p^2}{s^2 + 2\zeta\omega_p s + \omega_p^2}$ & 0.2 \\ 
\\[-0.5em]
case 5 & $\frac{s+\omega_i}{s}$ & $\frac{8760}{s^2+5.886s+7443}$ & 0 \\
\\[-1em]
\hline
\end{tabular}}
\end{table}

% While in Cases 1-3, $e_{bl}(t)$ have two zero-crossing points during the first period, so their frequency threshold for multiple resets can be determined by Theorem \ref{thm: Delta} and Remark \ref{rem: Lambda}.     
Figure \ref{fig:Delta_3RCSS} displays the $\Delta(\omega)$ of Cases 1-3 at various frequencies calculated using Theorem \ref{thm: Delta}. The existence of multiple-reset is indicated by $\Delta(\omega)>0$ in these RCSs. Based on the plots, we anticipate that the multiple-reset regions for Cases 1-3 are $(0,\ 0.16)$ Hz, $(0,\ 4.5)$ Hz, and $(0,\ 5.8)$ Hz, respectively.

Figure \ref{fig:r_e} show the numerical results of Cases 1-5, showing the number of resets at different input frequency. These results are consistent with results in Fig.\ref{fig:Delta_3RCSS} predicted by Theorem \ref{thm: Delta}. 
\begin{figure}[htp]
    %  \centering
    %  \subfloat[Case 1]{
     \begin{subfigure}{0.15\textwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/Delta_ci_1stplant.pdf}
         \caption{Case 1}
	\label{fig:c1}
     \end{subfigure}
     \begin{subfigure}{0.15\textwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/Delta_ci_spider.pdf}
         \caption{Case 2}
	\label{fig:C2}
     \end{subfigure}
     \begin{subfigure}{0.15\textwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/Delta_fore_spider.pdf}
         \caption{Case 3}
	\label{fig:c3}
     \end{subfigure}
    \caption{$\Delta(\omega)$ and $\Delta'(\omega)$ in Cases 1-3.}
    \label{fig:Delta_3RCSS}
    \end{figure}
    
\begin{figure}[htp]
	%	\missingfigure{RCsystem}
	\centerline{\includegraphics[width=\columnwidth]{figs/numer_ri_case1.pdf}}
	\caption{$r(t)$ and $e(t)$ of (a) Case 1, (b) Case 2, and (c) Case 3 in Simulink.}
	\label{fig:r_e}
\end{figure}
\begin{figure}[htp]
	%	\missingfigure{RCsystem}
	\centerline{\includegraphics[width=\columnwidth]{figs/numer_ri_case2.pdf}}
	\caption{$r(t)$ and $e(t)$ of (a) Case 1, (b) Case 2, and (c) Case 3 in Simulink.}
	\label{fig:r_e}
\end{figure}
\begin{figure}[htp]
	%	\missingfigure{RCsystem}
	\centerline{\includegraphics[width=\columnwidth]{figs/numer_ri_case3.pdf}}
	\caption{$r(t)$ and $e(t)$ of (a) Case 1, (b) Case 2, and (c) Case 3 in Simulink.}
	\label{fig:r_e}
\end{figure}

In practice, $t_1$ in \eqref{eq: t1} is larger than the true first reset instant defined as $\Bar{t}_1$, since $t_1$ is calculated based on the steady-state function, whereas the transient response is present at the beginning of the time series. However, taking the transient response into consideration for these examples will make the calculation process redundant. In Fig. \ref{fig:Delta_3RCSS}, we compare the $\Delta(\omega)$ calculated using $t_1$ with $\Delta'(\omega)$ derived by $\Bar{t}_1$ in three RCSs. We can see the zero-crossing points of $\Delta(\omega)$ and $\Delta'(\omega)$ have no big difference. Thus, we can use the frequency-domain tool based on $\Delta(\omega)$ to determine whether multiple resets will occur in a RCS in practice.
% and \eqref{eq: Lamdba(w)}. $\Delta'(\omega)= e'_2(\Bar{t}_1)$ will be discussed in the next section, 
% \begin{figure}[htp]
% 	%	\missingfigure{RCsystem}
% 	\begin{center}
% 	\centerline{\includegraphics[width=0.8\columnwidth]{figs/RCS_2ndPlant.pdf}}
% 	\caption{Block diagram of a RCS.}
% 	\label{fig:RCS_2p}
% 	\end{center}
% \end{figure}

According to Proposition \ref{rem: Lambda}, when the single input signal of the RCS is a process disturbance $d(t)$, $\Lambda(\omega) < 0$ indicates that there will be multiple-reset. Similar to the determination process of Theorem \ref{thm: Delta}, the coherence of Fig. \ref{fig:lambda_3RCS} with Fig. \ref{fig:r_e} shows the proficiency of Proposition \ref{rem: Lambda}.
\begin{figure}[htp]
     \centering
      \begin{subfigure}{0.15\textwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/Lambda_ci_1stplant.pdf}
        %  \caption{$\Lambda(\omega)$.}
	\label{fig:Lambda(w)}
     \end{subfigure}
     \begin{subfigure}{0.15\textwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/Lambda_ci_spider.pdf}
        %  \caption{$\Lambda(\omega)$.}
	\label{fig:Lambda(w)}
     \end{subfigure}
     \begin{subfigure}{0.15\textwidth}
         \centering
         \includegraphics[width=\columnwidth]{figs/Lambda_fore_spider.pdf}
        %  \caption{$\Lambda(\omega)$.}
	\label{fig:Lambda(w)}
     \end{subfigure}
    \caption{$\Lambda(\omega)$ in Cases 1-3.}
    \label{fig:lambda_3RCS}
    \end{figure}
 %    \begin{figure}[htp]
	% %	\missingfigure{RCsystem}
	% \centerline{\includegraphics[width=\columnwidth]{figs/d_e_condition.pdf}}
	% \caption{$d(t)$ and $e(t)$ of (a) Case 1, (b) Case 2, and (c) Case 3 in Simulink.}
	% \label{fig:r_e}
 %    \end{figure}

Figure \ref{fig:case4} shows the error signal $e(t)$ and base-linear error signal $e_{bl}(t)$ of a RCS to illustrate Remark \ref{rem: ebl_mrcs}. The system employs a Proportional Clegg Integrator controller (\cite{hosseinnia2013fractional}) with a base-linear transfer function of $\frac{57120}{s}+628.32$ and a plant with transfer function $\frac{1}{0.009s^2+s}$. The input signal is a sinusoidal reference input $r(t)=\sin (2\pi f t)$ with $f=20$ Hz. The results indicate the presence of four zero-crossings in $e_{bl}(t)$ during the first transient cycle, resulting in multiple-reset in the RCS.
     \begin{figure}[H]
	%	\missingfigure{RCsystem}
	\centerline{\includegraphics[width=\columnwidth]{figs/bad_design.pdf}}
	\caption{The input signal $r(t)$ (in black, solid), the error signal $e(t)$ (in red, solid), and the base-linear error signal $e_{bl}(t)$ (in black, dashed) of a reset control system. The green circles are utilised to indicate the zero-crossing points of $e_{bl}(t)$, while the blue circles are used to mark the reset instants of the RCS in one period.}
	\label{fig:case4}
    \end{figure}
     % \begin{figure}[htp]
    %  \centering
    %  \begin{subfigure}[b]{0.15\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{figs/r_e(0.01).pdf}
    %      \caption{$f = 0.01$ Hz}
    %      \label{fig:three sin x}
    %  \end{subfigure}
    %  \begin{subfigure}[b]{0.15\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{figs/f=0.16.pdf}
    %      \caption{$f = 0.16$ Hz}
    %      \label{fig:five over x}
    %  \end{subfigure}
    %  \begin{subfigure}[b]{0.15\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{figs/f=0.2.pdf}
    %      \caption{$f = 0.2$ Hz}
    %      \label{fig:five over x}
    %  \end{subfigure}
    % \caption{Case 1: $d(t)$ and $e(t)$ in Simulink.}
    % \label{fig:de1}
    % \end{figure}
    % \begin{figure}[htp]
    %  \centering
    %  \begin{subfigure}[b]{0.15\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{figs/d_e(1.5)_ci_spider.pdf}
    %      \caption{$f = 1.5$ Hz}
    %      \label{fig:three sin x}
    %  \end{subfigure}
    %  \begin{subfigure}[b]{0.15\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{figs/d_e(2.05)_ci_spider.pdf}
    %      \caption{$f = 2$ Hz}
    %      \label{fig:five over x}
    %  \end{subfigure}
    %  \begin{subfigure}[b]{0.15\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{figs/d_e(2.5)_ci_spider.pdf}
    %      \caption{$f = 2.5$ Hz}
    %      \label{fig:five over x}
    %  \end{subfigure}
    % \caption{Case 2: $d(t)$ and $e(t)$ in Simulink.}
    % \label{fig:de2}
    % \end{figure}
    % \begin{figure}[htp]
    %  \centering
    %  \begin{subfigure}[b]{0.15\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{figs/FORE_Spider_1.5d_e.pdf}
    %      \caption{$f = 1.5$ Hz}
    %      \label{fig:three sin x}
    %  \end{subfigure}
    %  \begin{subfigure}[b]{0.15\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{figs/FORE_Spider_1.87d_e.pdf}
    %      \caption{$f = 1.87$ Hz}
    %      \label{fig:five over x}
    %  \end{subfigure}
    %  \begin{subfigure}[b]{0.15\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{figs/FORE_Spider_2d_e.pdf}
    %      \caption{$f = 2$ Hz}
    %      \label{fig:five over x}
    %  \end{subfigure}
    % \caption{Case 3: $d(t)$ and $e(t)$ in Simulink.}
    % \label{fig:de3}
    % \end{figure}
% \begin{figure}[htp]
%      \centering
%      \begin{subfigure}{0.2\textwidth}
%          \centering
%          \includegraphics[width=\columnwidth]{figs/Delta(w).pdf}
%         %  \caption{$\Delta(\omega)$ and $\Delta'(\omega)$.}
% 	\label{fig:Delta(w)}
%      \end{subfigure}
%      \begin{subfigure}{0.2\textwidth}
%          \centering
%          \includegraphics[width=\columnwidth]{figs/Lambda(w).pdf}
%         %  \caption{$\Lambda(\omega)$.}
% 	\label{fig:Lambda(w)}
%      \end{subfigure}
%     \caption{$\Delta(\omega)$, $\Delta'(\omega)$, and $\Lambda(\omega)$ of the RCS.}
%     \label{fig:DL}
%     \end{figure}
% \begin{figure}[htp]
% 	%	\missingfigure{RCsystem}
% 	\centerline{\includegraphics[width=0.7\columnwidth]{figs/Delta(w).pdf}}
% 	\caption{$\Delta(\omega)$ and $\Delta'(\omega) = e'_2(\Bar{t}_1)$, where $\Bar{t}_1$ is the first reset instant calculated by considering the transient response.}
% 	\label{fig:Delta(w)}
% \end{figure}
% \begin{table}[hb]
% \begin{center}
% \caption{$\Delta(\omega)$}\label{tb:v(w)}
% \begin{tabular}{ccccccc}
% Frequency (Hz) & 0.01 & 0.1 & 0.16 & 0.17 & 0.2 & 0.3\\\hline
% $\Delta(\omega)$ & 1.99 & 0.91 & -0.01 & -0.15 & -0.53 & -1.54 \\ \hline
% \end{tabular}
% \end{center}
% \end{table}
% \begin{table}[htp]
% \caption{}
% \begin{center}
% \begin{tabular}{ccccccc}
% Frequency (Hz) & 0.01 & 0.1 & 0.16 & 0.17 & 0.2 & 0.3\\\hline
% $\Delta(\omega)$ & 1.99 & 0.91 & -0.01 & -0.15 & -0.53 & -1.54 \\ \hline
% \end{tabular}
% \end{center}\label{tbV}
% \end{table}



==> 0_4_Methodology.tex <==
\section{Frequency-domain Analysis for Parallel-Partial Reset Control Systems}
\label{sec:methodology1}
In this section, Theorems \ref{thm: Open-loop HOSIDF for PP-RCS} and \ref{thm: Closed-loop HOSIDF for PP-RCS} propose the HOSIDF for open-loop PP-RCSs. 
\subsection{Frequency response Analysis for open-loop Parallel-Partial Reset Controllers}
% The reset controller $\mathcal{C}$ \eqref{eq: State-Space eq of RC} is constructed based on the primitive CI block \cite{banos2012reset}, with matrices $A_R$, $B_R$, $C_R$, and $D_R$, as shown in the state-space block diagram of $\mathcal{C}$. 
% \begin{figure}[h]
% 	%	\missingfigure{RCsystem}
% 	\centerline{\includegraphics[width=0.9\columnwidth]{Figs/statespace_reset_control.pdf}}
% 	\caption{The state-space block diagram of the reset controller $\mathcal{C}$.}
% 	\label{fig:state-space block diagram of C}
% \end{figure}

% To initiate the frequency response analysis for the open-loop reset controller, we begin by analyzing the CI. The Generalized CI (GCI) is defined as a reset controller \eqref{eq: State-Space eq of RC} with $A_R=0$, $B_R = 1$, $C_R = 1$, $D_R = 0$, and $A_\rho = \gamma \in(-1,1)$, satisfying Assumption \ref{open-loop stability}. Lemma \ref{lem: CI MODEL} elucidates that the output of the GCI consists of the sum of its base-linear output and a square wave.
% % Note that uppercase letters are used to indicate the frequency-domain components, while lowercases denote time-domain ones as per convention.
% \begin{lem}(The frequency response analysis for the open-loop GCI)
% 	\label{lem: CI MODEL} 
% Consider a GCI subjected to a sinusoidal input signal $e(t) = |E_1|\sin (\omega t+\angle E_1),\ \angle E_1\in (-\pi,\pi]$ and a reset triggered signal $e_s(t) = |E_s|\sin (\omega t +\angle E_s),\ \angle E_s\in (-\pi,\pi]$. The reset instant is given by $t_i = (i\pi-\angle E_s)/\omega, \ i\in\mathbb{Z}^+$. The steady-state output signal of the GCI denoted by $u_{ci}(t)$ is expressed as
% 	\begin{equation}
% 		\label{eq: ci to square wave}
% 		u_{ci}(t) = u_{i}(t) + q_i(t),
% 	\end{equation}
%     where $u_i(t)$ is the base-linear (integral) output given by
%     \begin{equation}
%         u_{i}(t) = -|E_1/\omega|[\cos(\omega t+\angle E_1)-\cos(\angle E_1)].
%         % \begin{cases}
%    %     0, & \text{for even}\ i, \\
%    %     {2|E_1|}/{\omega}, & \text{for odd}\ i.
%    % \end{cases}  
%     \end{equation}
%     $q_i(t)$ is a $2\pi/\omega$-periodical square wave given by
% \begin{equation}
% 		\label{eq: q_i(t)final}
% 		q_i(t) = 
% 		\begin{cases}
% 			{\Delta_s(\omega) }/{(\gamma+1)}, & \text{for}\ t \in [t_{2k}, t_{2k+1}),\\
% 			{\gamma\Delta_s(\omega) }/{(\gamma+1)}+\\
%    (\gamma - 1)[\Delta_e(\omega)+\Delta_o(\omega)], &  \text{for}\ t \in [t_{2k+1}, t_{2k+2}),
% 		\end{cases}
% 	\end{equation}		
% where $k\in\mathbb{N}$.												
% \end{lem}
% \begin{proof} 
% The reset actions is triggered by the signal $e_s(t) =  |E_s|\sin (\omega t +\angle E_s)$. The set of the reset instants is defined as $J_{c} = \{t_i= (i\pi-\angle E_s)/\omega, \ i\in\mathbb{Z}^+\}$. The reset interval defined as $\delta_i=t_{i+1}-t_i=\pi/\omega$ is lower bounded. Thus, the outputs of the GCI is Zeno-free.

% Based on \eqref{eq: State-Space eq of RC}, the output signal $u_{ci}(t)$ of the GCI (with $A_R =0, B_R = 1, C_R = 1, D_R = 0$) is given by
% \begin{equation}
% \label{uci, t+}
% \begin{cases}
% \dot u_{ci}(t) = e(t), & t\notin J_c, \\
% u_{ci}(t^+) = \gamma u_{ci}(t), & t\in J_c.
% \end{cases}
% \end{equation}
% For its BLS (which is an integrator), we have 
% \begin{equation}
% \label{eq: dot ui}
%     \dot u_{i}(t) = e(t).
% \end{equation}
% Define $q_i(t) = u_{ci}(t) - u_{i}(t)$. From \eqref{uci, t+} and \eqref{eq: dot ui}, we have
% 	\begin{equation}
%  \label{eq: qi(t)0}
% 		\begin{cases}
% 			\dot q_i(t) = \dot u_{ci}(t) - \dot u_{i}(t) = 0, & t\notin J_c,\\
% 			q_i(t^+) = \gamma q_i(t) + (\gamma - 1)u_{i}(t), & t\in J_c.
% 		\end{cases}
% 	\end{equation}	
% From \eqref{eq: qi(t)0}, the signal $q_i(t)$ between two consecutive reset instants $[t_i^+, t_{i+1}]$ (where $t_i^+$ denotes the after-reset instant) is expressed as:
% 	\begin{equation}
% 		\label{eq: qi(t)1}
% 		q_i(t) = q_i(t_i^+) + \int_{t_i}^{t}\dot q_i(\tau)d\tau = q_i(t_i^+),\ t\in [t_i^+, t_{i+1}].
% 	\end{equation}
% The output signal of an integrator to a input signal of $e(t) = |E_1|\sin(\omega t +\angle E_1)$ is given by
% \begin{equation}
%  u_{i}(t) = -|E_1/\omega|[\cos(\omega t+\angle E_1)-\cos(\angle E_1)].   
% \end{equation}
% At the reset instant $t_i=t_i = (i\pi-\angle E_s)/\omega$, $u_i(t_i)$ is given by
% \begin{equation}
% \label{uti}
%    u_{i}(t_i) = \begin{cases}
%        |E_1/\omega|[\cos(\angle E_1)-\cos(\angle E_s-\angle E_1)], & \text{for even}\ i, \\
%         |E_1/\omega|[\cos(\angle E_1)+\cos(\angle E_s-\angle E_1)], & \text{for odd}\ i.
%    \end{cases} 
% \end{equation}
% Combining \eqref{eq: qi(t)0}, \eqref{eq: qi(t)1}, and \eqref{uti}, at the reset instant $t_i$, $q_i(t_i^+)$ is given by
% \begin{equation}
% \label{eq:qi00}
% \begin{split}
% % \begin{aligned}
% 		 q_i(t_i^+)&= \gamma q_i(t_{i-1}^+) + (\gamma - 1)u_{i}(t_i)\\
% 		&= \begin{cases}
% 			\gamma q_i(t_{i-1}^+)+|E_1/\omega|(\gamma - 1)*\\
%    [\cos(\angle E_1)-\cos(\angle E_s-\angle E_1)], & \text{for even}\ i, \\
% 			\gamma q_i(t_{i-1}^+) + |E_1/\omega|(\gamma - 1)*\\
%    [\cos(\angle E_1)+\cos(\angle E_s-\angle E_1)], & \text{for odd}\ i.
% 		   \end{cases}
% 	% \end{aligned}    
% \end{split}
% \end{equation}
% Based on \eqref{eq:qi00}, for an even $i$, $q_i(t_i^+)$ is given by 
% \begin{equation}
% \label{eq:qi01}
% 	\begin{aligned}
% 		q_i(t_i^+) &= q_i(t_{i+2}^+)\\
% 		&= 	\gamma q_i(t_{i+1}^+) +|E_1/\omega|(\gamma - 1)*\\
%   &\indent\indent\indent [\cos(\angle E_1)-\cos(\angle E_s-\angle E_1)]\\
% 		&= 	\gamma^2 q_i(t_{i}^+) + |E_1/\omega|\gamma(\gamma - 1)*\\
%   &\indent\indent\indent [\cos(\angle E_1)+\cos(\angle E_s-\angle E_1)]+\\
%   &\indent\indent\indent |E_1/\omega|(\gamma - 1)[\cos(\angle E_1)-\cos(\angle E_s-\angle E_1)]\\
%   &= \gamma^2 q_i(t_{i}^+) + |E_1/\omega|[(\gamma^2 - 1)*\\
%   &\indent\indent\indent \cos(\angle E_1)+(\gamma - 1)^2\cos(\angle E_s-\angle E_1)].
% 	\end{aligned}
% \end{equation}
% From \eqref{eq:qi01}, for an even $i$, $q_i(t_i^+)$ is given by
% \begin{equation}
% \label{q_i+,even}
% q_i(t_i^+) = {\Delta_s(\omega) }/{(\gamma+1)},   
% \end{equation}
% where 
% \begin{equation}
% \label{eq: Delta_s,e,o}
% \begin{aligned}
% \Delta_s(\omega) &= -[(\gamma+ 1)\Delta_e(\omega) + (\gamma - 1)\Delta_o(\omega)],\\ 
% \Delta_e(\omega) &= |E_1/\omega|\cos(\angle E_1),\\
% \Delta_o(\omega) &= |E_1/\omega|\cos(\angle E_s-\angle E_1).
% \end{aligned}
% \end{equation}
% From \eqref{eq:qi00}, \eqref{q_i+,even}, and \eqref{eq: Delta_s,e,o}, for an odd $i$, $q_i(t_i^+)$ is given by
% \begin{equation}
% \label{q_i+,odd}
% q_i(t_i^+) = {\gamma\Delta_s(\omega) }/{(\gamma+1)}+(\gamma - 1)[\Delta_e(\omega)+\Delta_o(\omega)].   
% \end{equation}
% From \eqref{eq: qi(t)1}, \eqref{q_i+,even}, and \eqref{q_i+,odd}, $q_i(t)$ in the time domain can be derived as follows:
% 	\begin{equation}
% 		\label{eq: q(t)00}
% 		q_i(t) = 
% 		\begin{cases}
% 			{\Delta_s(\omega) }/{(\gamma+1)}, & \text{for}\ t \in [t_{2k}, t_{2k+1}),\\
% 			{\gamma\Delta_s(\omega) }/{(\gamma+1)}+\\
%    (\gamma - 1)[\Delta_e(\omega)+\Delta_o(\omega)], &  \text{for}\ t \in [t_{2k+1}, t_{2k+2}).
% 		\end{cases}
% 	\end{equation}	
% Here we conclude the proof.
% \end{proof}
% Define 
% \begin{equation}
% \mathcal{C}_{\rho}^n(\omega) = H_n(\omega)-C_{bl}(\omega).    
% \end{equation}
% From \eqref{eq: RL} and \eqref{eq: HOSIDF}, $\mathcal{C}_{\rho}^n(\omega)$ is given by
% \begin{equation}
% \label{eq: Cnl}
% \begin{aligned}
% \mathcal{C}_{\rho}^n(\omega)=C_R(jn\omega I-A_R)^{-1}j\Theta _D(\omega)B_R,
% \end{aligned}
% \end{equation}
% where $n = 2k+1, k\in\mathbb{N}$.
\begin{thm} (The Higher-order sinusoidal input describing function (HOSIDF) for the parallel-partial reset controller (PP-RC))
\label{thm: Open-loop HOSIDF for PP-RCS}
Consider a parallel-partial reset controller (PP-RC) $\mathcal{H}_p$ as depicted in Fig. \ref{fig1:PP-RC system}, operating under the sinusoidal input signal $e_1(t) = |E_1|\sin (\omega t + \angle E_1)$, where $\angle E_1\in[-\pi,\pi)$, and under the Assumption \ref{open-loop stability}. The steady-state output signal of $\mathcal{H}_p$ is denoted as $v_1(t)$, which comprises $n$ harmonics, represented as $v_1(t) = \sum\nolimits_{n=1}^{\infty}v_{1n}(t)$, where $n=2k+1$ and $k\in\mathbb{N}$. The block diagram of $\mathcal{H}_p$ is illustrated in Fig. \ref{fig1:PP-RC system2}. By utilizing the ``Virtual Harmonic Generator" \cite{saikumar2021loop}, the input signal $e_1(t)$ generates $n$ harmonics, denoted as $e_{1n}(t) = |E_1|\sin (n\omega t + n\angle E_1)$. The $n$-th Higher-Order Sinusoidal Input Describing Function (HOSIDF) for $\mathcal{H}_p$, defined as $H_{p}^n(\omega)$, represents the transfer function from $E_{1n}(\omega) = \mathscr{F}[e_{1n}(t)]$ to $V_{1n}(\omega) = \mathscr{F}[v_{1n}(t)]$, and is given by:
    \begin{equation}
    \label{eq: H_{p}^n}
    H_{p}^n(\omega) = \frac{V_{1n}(\omega)}{E_{1n}(\omega)}=
        \begin{cases}
	 	\mathcal{C}_{bl}(\omega) + k_{rc} \mathcal{C}_{\rho}^1(\omega), & \text{for } n=1\\
	 	k_{rc} \mathcal{C}_{\rho}^n(\omega), & \text{for odd} \ n > 1\\
	 	0, & \text{for even} \ n \geqslant 2 
        \end{cases}
    \end{equation}
    where $\mathcal{C}_{bl}(\omega)$ is given in \eqref{eq: RL} and $\mathcal{C}_{\rho}^n(\omega)$ is given by
    \begin{equation}
    \label{eq: C_rho_n}
     \mathcal{C}_{\rho}^n(\omega) = C_R(jn\omega I-A_R)^{-1}j\Theta _D(\omega)B_R,  
    \end{equation}
    in which $\Theta _D(\omega)$ is given in \eqref{Theta_D}.
   \begin{figure}[h]
	%	\missingfigure{RCsystem}
	\centerline{\includegraphics[width=0.9\columnwidth]{Figs/Partial RCS3.pdf}}
	\caption{The block diagram of the parallel-partial reset controller (PP-RC), where $e_1(t)$ and $v_1(t)$ are the input and output signals.}
	\label{fig1:PP-RC system2}
\end{figure}
\end{thm}
\begin{proof}
The HOSIDF for a reset controller $\mathcal{C}$ is $H_n(\omega)$ given in \eqref{eq: HOSIDF}. 
Define 
\begin{equation}
\begin{aligned}
\label{eq: Cro defn}
\mathcal{C}_{\rho}^1(\omega) &= H_1(\omega) -\mathcal{C}_{bl}(\omega), \\
\mathcal{C}_{\rho}^n(\omega) &= H_n(\omega), \text{ for }n>1.
\end{aligned}
\end{equation}
From \eqref{eq: HOSIDF} and \eqref{Theta_D}, the expression for $\mathcal{C}_{\rho}^n(\omega)$ is given in \eqref{eq: C_rho_n}. 

From \eqref{eq: Hpp} and \eqref{eq: Cro defn}, the $n$-th HOSIDF for $\mathcal{H}_{rc}$ is given by
\begin{equation}
\label{eq: H_{rc}^n}
\mathcal{H}_{rc}^n(\omega) =
\begin{cases}
k_{rc} \mathcal{C}_{bl}(\omega) + k_{rc} \mathcal{C}_{\rho}^1(\omega), & \text{for } n=1\\
k_{rc} \mathcal{C}_{\rho}^n(\omega), & \text{for odd} \ n > 1\\
0, & \text{for even} \ n \geqslant 2 
\end{cases}
\end{equation}
The transfer function for $\mathcal{H}_{bl}$ is 
\begin{equation}
\label{eq: Hbl(w)}
\mathcal{H}_{bl}(\omega) =  (1-k_{rc})\mathcal{C}_{bl}(\omega).  
\end{equation}
Substituting \eqref{eq: H_{rc}^n} and \eqref{eq: Hbl(w)} into \eqref{eq: Hpp}, the $n$-th HOSIDF for $\mathcal{H}_{p}$ is derived as shown in \eqref{eq: H_{p}^n}. The proof is concluded.
\end{proof}
% Figure \ref{fig1: Valid_PP-PCI_OL} showcases the open-loop Bode plot of the \enquote{PI+CI} control structure, with parameter values $(k_{rc}, \gamma) = (0.5, -0.7)$. The plot is generated using our novel HOSIDF approach in \eqref{eq: H_{p}^n}, and it's comparison against results obtained from state-space calculations as per the literature \cite{banos2007definition}.

% The comparison demonstrates that our new method aligns seamlessly with the existing techniques. An important distinction, however, is that our method isn't restricted solely to the \enquote{PI+CI} structure; it's applicable to a broader class of PP-RCSs. Furthermore, it offers fresh insights into the frequency-domain analysis of open-loop PP-RCSs by effectively separating the linear and nonlinear components. This deeper understanding will aid for forthcoming frequency-domain analysis for closed-loop PP-RCSs.
% \begin{figure}[htp]
% 	%	\missingfigure{RCsystem}
% 	\centerline{\includegraphics[width=\columnwidth]{Figs/Valid_PP-PCI_OL.pdf}}
% 	\caption{Bode plot of \enquote{PI+CI} controller, showing the first ($L_1(\omega)$) and third ($L_3(\omega)$) harmonics obtained from \cite{banos2007definition}, alongside the first ($H_{PP1}(\omega)$) and third ($H_{PP3}(\omega)$) harmonics obtained from equation \eqref{eq: H_{p}^n}.}
% 	\label{fig1: Valid_PP-PCI_OL}
% \end{figure}

\subsection{Frequency-domain Analysis for closed-loop Parallel-Partial Reset Control Systems}
\begin{prop}
Consider a reset controller $\mathcal{C}$ takes a sinusoidal input signal $e(t) = |E_n|\sin(n\omega t + \angle E_n)\ (\angle E_s\in (-\pi,\pi],\ n=2k+1,\ k\in\mathbb{N})$ and a $2\pi/\omega$-periodic reset triggered signal denoted by $e_s(t) = |E_s|\sin(\omega t+\angle E_s),\ (\angle E_s\in (-\pi,\pi])$, under Assumption \ref{open-loop stability}. The state $x_r(t)$ is given by
	\begin{equation}
		\label{eq: vbl}
		x_{r}(t) = x_{bl}(t) + x_{nl}(t),
	\end{equation}    
 where $x_{bl}(t)$ is the base-linear state given by
 \begin{equation}
 \begin{aligned}
      \Delta_l(n\omega) &= (jn\omega I-A_R)^{-1}B_R,\\
     x_{bl}(t) &= |E_n\Delta_l(n\omega) |\sin(n\omega t+ n\angle E_n+\angle \Delta_l(n\omega) ).
 \end{aligned}
 \end{equation}
 $x_{nl}(t)$ is a nonlinear signal that has the same phase with the reset triggered signal $e_s(t)$, given by
 \begin{equation}
\label{eq: DELTAN FINAL}
    x_{nl}(t) = 
    \begin{cases}
     |E_1|e^{A_R (t-t_i)}\Delta_v^n(\omega),\ &\text{for even }i,\\
     -|E_1|e^{A_R (t-t_i)}\Delta_v^n(\omega),\ &\text{for odd }i,    
    \end{cases}
\end{equation}
where 
\begin{equation}
\label{eq: Delta_v}
\Delta_v^n(\omega) =(A_\rho e^{A_R\pi/\omega}-I)^{-1}(I-A_\rho)\Delta_c^n(\omega).    
\end{equation}
\end{prop}
\begin{proof}
Consider a reset controller $\mathcal{C}$ \eqref{eq: State-Space eq of RC} with an input signal of $e(t) = |E_n|\sin(n\omega t + \angle E_n)\ (n=2k+1,\ k\in\mathbb{N})$ and a reset triggered signal of $e_s(t) = |E_s|\sin(\omega t+\angle E_s), \ (-\pi<\angle E_s<\pi)$. The set of reset instants is denoted by $J_o := \{t_i = (i\pi-\angle E_s)/\omega \mid i \in \mathbb{Z}^{+}\}$. The reset interval is given by $\delta_i = t_{i+1}-t_i=\pi/\omega$.    

Let $x_c(t)$ and $x_{bl}(t)$ denote the state and the base-linear state of the $\mathcal{C}$ and the BLC $\mathcal{C}_{bl}$, respectively. Define
\begin{equation}
\label{A: eq: xc,xnl,xbl}
    x_{nl}(t) = x_c(t) - x_{bl}(t),
\end{equation}
where $n_c$ is the number of states of the reset controller $\mathcal{C}$ and $x_{bl}(t)$ is given by
\begin{equation}
\label{A: X_bl(t)npi}
    x_{bl}(t) = |E_n\Delta_l(n\omega)|\sin(n\omega t + \angle E_n + \angle\Delta_l(n\omega)),
\end{equation}
where 
\begin{equation}
 \Delta_l(n\omega) = (jn\omega I-A_R)^{-1}B_R.   
\end{equation}
Based on \eqref{eq: State-Space eq of RC} and \eqref{A: eq: xc,xnl,xbl}, we have:
\begin{equation}
\label{A: eq: q(t)11}
    \begin{cases}
        \dot x_{nl}(t) = A_Rx_{nl}(t), &  t\notin J_o,\\
        x_{nl}(t^+) = A_\rho x_{nl}(t) + (A_\rho-I)x_{bl}(t), & t\in J_o.
    \end{cases}
\end{equation}
According to \eqref{A: eq: q(t)11}, between two consecutive reset instants $[t_{i}^+, t_{i+1}]$ where $e_s(t) \neq 0$, the expression for $x_{nl}(t)$ is given by
\begin{equation}
\label{A: xnl(t)}
    x_{nl}(t) = e^{A_R (t-t_i)}\Delta_n(\omega) , \ \text{ for } t\in[t_{i}^+, t_{i+1}],
\end{equation}
where $\Delta_n(\omega)\in \mathbb{R}^{n_c\times 1}$ is a constant matrix independent of time $t$.

Based on \eqref{A: xnl(t)}, at the reset instant $t_{i+1} \in J_o$, $x_{nl}(t_{i+1})$ is given by
\begin{equation}
\label{A: xnl(t_i+1)}
    x_{nl}(t_{i+1}) = e^{A_R (t_{i+1}-t_i)}\Delta_n(\omega)  =e^{A_R\pi/\omega} \Delta_n(\omega) .
\end{equation}
From \eqref{A: eq: q(t)11}, $x_{nl}(t^+)$ at the reset instant $t_{i+1}$ is given by
\begin{equation}
\label{A: xnl(t_i+1+)}
    x_{nl}(t_{i+1}^+) = A_\rho x_{nl}(t_{i+1}) + (A_\rho-I)x_{bl}(t_{i+1}).
\end{equation}
Substituting $x_{nl}(t_{i+1})$ from \eqref{A: xnl(t_i+1)} into \eqref{A: xnl(t_i+1+)}, $x_{nl}(t_{i+1}^+)$ is obtained as
\begin{equation}
\label{A: xnl(t_i+1+)2}
    x_{nl}(t_{i+1}^+)  = A_\rho e^{A_R\pi/\omega} \Delta_n(\omega) + (A_\rho-I)x_{bl}(t_{i+1}).
\end{equation}
From \eqref{A: X_bl(t)npi}, at the reset instant $t_i= (i\pi-\angle E_s)/\omega$, the base-linear state is given by
\begin{equation}
\label{A: eq:x_bl(t_i)_npi0}
x_{bl}(t_i) = |E_n\Delta_l(n\omega)|\sin(ni\pi+ \angle E_n + \angle\Delta_l(n\omega)-n\angle E_s).   
\end{equation}
Equation \eqref{A: eq:x_bl(t_i)_npi0} is written as
\begin{equation}
\label{A: eq:x_bl(t_i)_npi}
\begin{aligned}
   &x_{bl}(t_i) =\\
    &\begin{cases}
        |E_n\Delta_l(n\omega)|\sin(\angle\Delta_l(n\omega)+ \angle E_n-n\angle E_s), & \text{ for even }i,\\
        -|E_n\Delta_l(n\omega)|\sin(\angle\Delta_l(n\omega)+ \angle E_n-n\angle E_s), & \text{ for odd }i.
    \end{cases}
\end{aligned}
\end{equation}
Define 
\begin{equation}
\label{A: eq: Delta_cn}
\Delta_c^n(\omega) = |\Delta_l(n\omega)|\sin(\angle\Delta_l(n\omega)+ \angle E_n-n\angle E_s),   
\end{equation}
and substitute $\Delta_c^n(\omega)$ from \eqref{A: eq: Delta_cn} into \eqref{A: eq:x_bl(t_i)_npi}, we have
\begin{equation}
\label{A: eq:x_bl(t_i)_npi2}
    x_{bl}(t_i) = 
    \begin{cases}
        |E_n|\Delta_c^n(\omega), & \text{ for even }i,\\
        -|E_n|\Delta_c^n(\omega), & \text{ for odd }i.
    \end{cases}    
\end{equation}
From \eqref{A: eq:x_bl(t_i)_npi2}, at the reset instant $t_{i+1} = ((i+1)\pi-\angle E_s)/\omega$, the expression for $x_{bl}(t_{i+1})$ is written as:
\begin{equation}
\label{A: eq:xbl(ta+)1}
    x_{bl}(t_{i+1}) =
    \begin{cases}
    -|E_n|\Delta_c^n(\omega),\ &\text{for even }i,\\
    |E_n|\Delta_c^n(\omega),\ &\text{for odd }i,  
    \end{cases}    
\end{equation}
Substituting $x_{bl}(t_{i+1})$ from \eqref{A: eq:xbl(ta+)1} into \eqref{A: xnl(t_i+1+)2}, $x_{nl}(t_{i+1}^+)$ is derived as
\begin{equation}
\label{A: eq:xnl(ta+)0}
\begin{aligned}
    &x_{nl}(t_{i+1}^+) =\\
    &\begin{cases}
    A_\rho e^{A_R\pi/\omega}\Delta_n(\omega)  - (A_\rho-I)|E_n|\Delta_c^n(\omega),\ &\text{for even }i,\\
    A_\rho e^{A_R\pi/\omega}\Delta_n(\omega)  + (A_\rho-I)|E_n|\Delta_c^n(\omega),\ &\text{for odd }i.   
    \end{cases}    
\end{aligned}
\end{equation}
From \eqref{A: eq:xnl(ta+)0}, we have
\begin{equation}
\label{A: eq:xnl(ta+)}
\begin{aligned}
    &x_{nl}(t_{i}^+) =\\
    &\begin{cases}
    A_\rho e^{A_R\pi/\omega}\Delta_n(\omega)  + (A_\rho-I)|E_n|\Delta_c^n(\omega),\ &\text{for even }i,\\
    A_\rho e^{A_R\pi/\omega}\Delta_n(\omega)  - (A_\rho-I)|E_n|\Delta_c^n(\omega),\ &\text{for odd }i.  
    \end{cases}   
\end{aligned}
\end{equation}
From \eqref{A: xnl(t)}, at the reset instant $t_i^+$, we have
\begin{equation}
\label{A: x_nl_ti+}
    x_{nl}(t_i^+) = \Delta_n(\omega).
\end{equation}
Let equations \eqref{A: eq:xnl(ta+)} and \eqref{A: x_nl_ti+} be set equal to each other. Then, $\Delta_n(\omega)$ is derived as follows:
\begin{equation}
\label{A: eq:xnl(ta+)2}
    \Delta_n(\omega) = 
    \begin{cases}
     |E_n|\Delta_v^n(\omega),\ &\text{for even }i,\\
     -|E_n|\Delta_v^n(\omega),\ &\text{for odd }i,   
    \end{cases}
\end{equation}
where 
\begin{equation}
\label{A: eq: Delta_vn}
    \Delta_v^n(\omega) = (A_\rho e^{A_R\pi/\omega}-I)^{-1}(I-A_\rho)\Delta_c^n(\omega).
\end{equation}
Since $\delta_i=\pi/\omega$, equations \eqref{A: xnl(t)} and \eqref{A: eq:xnl(ta+)2} together illustrate that $x_{nl}(t)$ has the same period as the reset triggered signal $e_s(t)$.
\end{proof}
% Given a complex function $f$, $f\in \mathscr{L}_2$ on time axis $[0,\infty]$ if $f$ is (Lebesgue) measurable and if
% \begin{equation}
%     \int_{0}^{\infty} |f|^2 \,du < +\infty. 
% \end{equation}
% In this way, $f$ is square-integrable.
Stability and convergence are crucial for the existence of steady-state solutions, enabling frequency response analysis. While the primary focus is on developing the steady-state response, stability and convergence are fundamental aspects that can be achieved through proper design. To ensure stability and convergence, we make the following assumptions based on existing literature:
\begin{assum}
\label{assum: stable}
The closed-loop reset control system is assumed to satisfy the following conditions: the initial condition of the reset controller $\mathcal{C}$ is zero, the reset system is asymptotically stable \cite{banos2012reset}, there are infinitely many reset instants $t_i$ with $\lim_{t_i \to \infty} = \infty$, the input signal $r(t) = |R|\sin(\omega t)$ is a Bohl function, \cite{barabanov2001bohl}, and there is no Zenoness behaviour.
\end{assum}

Under Assumption \ref{assum: stable}, as per \cite{pavlov2006uniform}, $e(t)$, $v(t)$, $u(t)$, and $y(t)$ are periodic signals with the same fundamental frequency as $r(t)$ and can be expressed as follows:
\begin{equation}
\label{eq: e,y,u}
    \begin{aligned}
        e(t) &= \sum\nolimits_{n=1}^{\infty}e_n(t) = \sum\nolimits_{n=1}^{\infty} |E_n|\sin(n\omega t+\angle E_n),\\
        v(t) &= \sum\nolimits_{n=1}^{\infty}v_n(t) = \sum\nolimits_{n=1}^{\infty} |V_n|\sin(n\omega t+\angle V_n),\\
        u(t) &= \sum\nolimits_{n=1}^{\infty}u_n(t) = \sum\nolimits_{n=1}^{\infty} |U_n|\sin(n\omega t+\angle U_n),\\
        y(t) &= \sum\nolimits_{n=1}^{\infty}y_n(t) = \sum\nolimits_{n=1}^{\infty} |Y_n|\sin(n\omega t+\angle Y_n), 
    \end{aligned}
\end{equation}
where $e_n(t)$, $v_n(t)$ , $u_n(t)$ and $y_n(t)$ are their n$^{\text{th}}$ harmonics, whose Fourier transformations are defined as $E_{n}(n\omega)$, $U_{n}(n\omega)$ and $Y_{n}(n\omega)$, respectively.

In the literature, multiple reset actions introduce more higher-order harmonics to the system compared to systems with only two reset actions \cite{saikumar2021loop}, which can be mitigated through careful design considerations \cite{karbasizadeh2020band}. Additionally, it is observed that most practical reset control systems are implemented with two reset actions \cite{BANOS2022101259}. Based on these insights, we introduce the following assumption.
\begin{assum}
\label{assum:2reset}
     There are two reset instants in a SISO closed-loop reset control system with a sinusoidal reference input signal $r(t) = |R|\sin(\omega t)$ at steady-state, where the reset-triggered signal is $e_1(t)$. 
\end{assum}
Under Assumptions \ref{assum: stable} and \ref{assum:2reset}, the reset actions in the closed-loop SISO reset control system occur when $e_{1}(t) = |E_1|\sin(\omega t + \angle E_1)= 0$, where $\angle E_1\in(-\pi,\pi]$. The set of reset instants for this closed-loop reset system is denoted as $J_m := \{t_m = (m\pi - \angle E_1)/\omega | m \in \mathbb{Z}^+\}$. Since the reset interval $\delta_m = t_{m+1}-t_m = \pi/\omega> \delta_{\text{min}}$, \cite{barreiro2014reset} the trajectories for the reset system are Zeno-free.
\begin{thm} 
\label{thm: Closed-loop HOSIDF for PP-RCS}
(Closed-loop HOSIDF for PP-RCSs) Under Assumptions \ref{assum: stable} and \ref{assum:2reset}, the n$^{\text{th}}$ sensitivity function $\mathcal{S}_n(n\omega)$ of a SISO PP-RCS in closed-loop in Fig. \ref{fig1:PP-RC system} with a sinusoidal reference signal $r(t) = R_0\sin(\omega t)$ (with $\mathscr{F}[r(t)] = R(\omega)$) at steady-states is defined as  
 \begin{equation}
	 	\label{eq: sensitivity functions in CL1}
   \begin{aligned}
	\mathcal{S}_n(n\omega)&= \frac{E_n(\omega)}{R_n(\omega)}\\
	   &=\begin{cases}
	 	\frac{1}{1+\mathcal{L}_{o}(\omega)} , & \text{for } n=1\\
	 	-\frac{\Gamma(\omega)\mathcal{L}_{nl}(n\omega)|\mathcal{S}_{1}(\omega)|e^{jn\angle \mathcal{S}_{1}(\omega)}}{1+\mathcal{L}_{bl}(n\omega)} , & \text{for odd} \ n > 1\\
	0, & \text{for even} \ n \geqslant 2 \end{cases}       
   \end{aligned}
	 \end{equation}
  where
 \begin{equation}
\label{eq: Gamma for PP-RCS}
\begin{aligned}
\mathcal{L}_{bl}(n\omega) &= \mathcal{C}_{bl}(n\omega)\mathcal{C}_{2}(n\omega)\mathcal{P}(n\omega),\\
\mathcal{L}_{o}(n\omega) &= \mathcal{L}_{bl}(n\omega) + \Gamma(\omega)\mathcal{L}_{nl}(n\omega),\\
\mathcal{L}_{nl}(n\omega) &= k_{rc}\mathcal{C}_{nl}(n\omega)\mathcal{C}_{2}(n\omega)\mathcal{P}(n\omega),\\
\zeta(n\omega) &= {|\mathcal{L}_{nl}(n\omega)|}/{|1+\mathcal{L}_{bl}(n\omega)|},\\
\eta_1(\omega) &= -k_{rc}\lvert\mathcal{C}_{bl}(\omega)\rvert \sin(\angle \mathcal{C}_{bl}(\omega)),\\
\Gamma(\omega) &= 1/[1-{\sum\nolimits_{n=3}^{\infty}\zeta(n\omega)\eta_n(\omega)}/{\eta_1(\omega)}],\\
\eta_n(\omega) &= k_{rc}|\mathcal{C}_{bl}(n\omega)| \sin(\angle\mathcal{L}_{nl}(n\omega)-\angle (1+\\
&\indent\indent\indent\indent\indent \indent\indent \mathcal{L}_{bl}(n\omega)) + \angle \mathcal{C}_{bl}(n\omega)).
		\end{aligned}
	\end{equation}   
\end{thm}
\begin{proof}
% Based on \eqref{eq: H_rc}, the n$^{\text{th}}$ open-loop linear and nonlinear transfer functions for each input signal $e_n(t)$ in \eqref{eq: e,y,u} are given by
% \begin{equation}
%     \begin{aligned}
%         \mathcal{L}_{bl}(n\omega) &= \mathcal{C}_{bl}(n\omega)\mathcal{C}_{2}(n\omega)\mathcal{P}(n\omega),\\
%         \mathcal{L}_{nl}(n\omega) &= k_{rc}\sum\nolimits_{n=1}^{\infty}\mathcal{C}_{\rho}^n(\omega)\mathcal{C}_{2}(n\omega)\mathcal{P}(n\omega).
%     \end{aligned}
% \end{equation}
The error signal $e(t)$ in the closed-loop PP-RCS, as defined in \eqref{eq: e,y,u}, comprises multiple harmonics ($n$ harmonics). Each harmonic component, denoted as $e_n(t)$, passes through the transfer function $\mathcal{H}_{p}$ to generate its respective output signal $v_n(t)$. According to Theorem \ref{thm: Open-loop HOSIDF for PP-RCS}, $v_1(t)$ consists of both a linear component, $v_{bl1}(t)$, and a nonlinear component, $v_{nl1}(t)$, expressed as follows:
\begin{equation}
\label{eq:v,vnl,vbl}
\begin{aligned}    
    v_1(t) &= v_{bl1}(t) + v_{nl1}(t),\\
    v_{bl1}(t) & = \mathscr{F}^{-1}\bigg[E_1(n\omega) \mathcal{C}_{bl}(n\omega)\bigg],\\
    v_{nl1}(t) & = k_{rc}\cdot\mathscr{F}^{-1}\bigg[\sum\nolimits_{n=1}^{\infty}E_{1}(n\omega) \mathcal{C}_{\rho}^n(\omega)\bigg].    
\end{aligned}
\end{equation}
Under the Assumption \ref{assum: TwoReset}, each $e_n(t)$ resets based on one signal $e_1(t)$. Thus, the nonlinear outputs $v_{nln}(t)$ for each input harmonics $e_n(t)$ shares the same phase but varying magnitudes. We define the function $\Gamma(\omega)$ as follows:
\begin{equation}
\label{eq: Gamma_defn}
    \Gamma(\omega) = \frac{\sum\nolimits_{n=1}^{\infty}v_{nln}(t)}{v_{nl1}(t)}.
\end{equation}
Based on \eqref{eq: H_pp2}, the n$^{\text{th}}$ output $V_n(n\omega)$ of $\mathcal{H}_{p}$ consists of two elements: the n$^{\text{th}}$ harmonic $V_{bln}(n\omega)$ and $V_{nln}(n\omega)$, respectively, given by
\begin{equation}
\label{eq:Vn}
    V_n(n\omega) = V_{bln}(n\omega) + V_{nln}(n\omega).
\end{equation}
Combining \eqref{eq: H_pp2}, \eqref{eq:v,vnl,vbl}, and \eqref{eq: Gamma_defn}, $V_{bln}(\omega)$ and $V_{nln}(\omega)$ are given as
\begin{equation}
\label{eq: unln}
    \begin{aligned}
        V_{bln}(\omega) &= E_{1n}(n\omega)\mathcal{C}_{bl}(n\omega),\\
        V_{nln}(\omega) &= k_{rc}\Gamma(\omega)\sum\nolimits_{n=1}^{\infty}E_{1n}(n\omega)\mathcal{C}_{\rho}^n(\omega).
    \end{aligned}
\end{equation} 
Based on \eqref{eq:Vn} and \eqref{eq: unln}, $V_n(n\omega)$ is given by
\begin{equation}
\label{eq: Un}
    V_n(n\omega) = E_{1n}(n\omega)\bigg[C_{bl}(n\omega) + k_{rc}\Gamma(\omega)\sum\nolimits_{n=1}^{\infty}\mathcal{C}_{\rho}^n(\omega)\bigg].
\end{equation}
For the n$^{\text{th}}$ harmonic in the closed-loop, we have 
\begin{equation}
\label{eq:E_n}
\begin{aligned}
    E_n(\omega) &= - E_n(\omega)\mathcal{L}_{bl}(n\omega) - k_{rc}\Gamma(\omega)E_{1n}(n\omega)\mathcal{L}_{nl}(n\omega).
\end{aligned}
\end{equation}
where
\begin{equation}
\label{eq:Lbl,Lnl}
    \begin{aligned}
    \mathcal{L}_{bl}(n\omega) &= \mathcal{C}_{bl}(n\omega) \mathcal{C}_2(n\omega) \mathcal{P}(n\omega),\\
    \mathcal{L}_{nl}(n\omega) &= k_{rc}\mathcal{C}_{\rho}^n(\omega) \mathcal{C}_2(n\omega) \mathcal{P}(n\omega).
    \end{aligned}
\end{equation}
Based on $e_n(t)$ from \eqref{eq: e,y,u} and $e_{1n}(t)$ from \eqref{eq:e_1n}, we transfer \eqref{eq:E_n} to the Fourier-domain as follows:
\begin{equation}
\label{eq:phase and Mag}
\begin{aligned}
&|E_n||1+\mathcal{L}_{bl}(n\omega)| \sin(n\omega t + \angle E_n + \angle (1+\mathcal{L}_{bl}(n\omega))) = \\
&-\Gamma(\omega)|E_1||\mathcal{L}_{nl}(n\omega)| \sin(n\omega t + n\angle E_1 + \angle\mathcal{L}_{nl}(n\omega)).
\end{aligned}
\end{equation}
From \eqref{eq:phase and Mag} and because $|E_n|\geq0$, we obtain the following equations:
\begin{equation}
\label{eq: phase and Mag2}
    \begin{cases}
       |E_n| &=  \frac{\Gamma(\omega)|\mathcal{L}_{nl}(n\omega)|}{|1+\mathcal{L}_{bl}(n\omega)|}|E_1|,\\
       \angle E_n &= \pi+ n\angle E_1 + \angle\mathcal{L}_{nl}(n\omega) - \angle (1+\mathcal{L}_{bl}(n\omega)),
    \end{cases}
\end{equation}
where $n>1$.

Based on \eqref{eq: State-Space eq of RC}, at reset instant $t_i$, we have 
\begin{equation}
\label{eq: q_oln}
 v_{nl1}(t_i^+) = (\gamma-1 )v_{bl1}(t_i).
 \end{equation}
Based on \eqref{eq:v,vnl,vbl}, we have 
 \begin{equation}
 \label{eq:ul1_t}
 \begin{aligned}
     v_{bl1}(t_i) &= \mathscr{F}^{-1}[E_{1}(\omega)C_{bl}(\omega)]\lvert_{t_i}\\
     &= |E_1|\lvert \mathcal{C}_{bl}(\omega)\rvert \sin(i\pi + \angle \mathcal{C}_{bl}(\omega)).
\end{aligned}
 \end{equation}
Combining \eqref{eq: q_oln} and \eqref{eq:ul1_t}, $v_{nl1}(t_i^+)$ is given by
\begin{equation}
\label{eq:unl1_t}
    v_{nl1}(t_i^+) = (\gamma-1)|E_1|\lvert \mathcal{C}_{bl}(\omega)\rvert \sin(i\pi + \angle \mathcal{C}_{bl}(\omega)).
\end{equation} 
At reset instant $t_i^+$, we have
\begin{equation}
	\label{eq: q_oln1}
	\begin{aligned}
 v_{nln}(t_i^+) &= (\gamma-1 )v_{bln}(t_i)=(\gamma-1)|E_n||\mathcal{C}_{bl}(n\omega)|\cdot \\
  &\ \ \ \ \ \ \ \sin(in\pi + \angle E_n-n\angle E_1 +\angle \mathcal{C}_{bl}(n\omega)).
	\end{aligned}
\end{equation}
Substitute $\angle E_n$ in \eqref{eq: phase and Mag2} to \eqref{eq: q_oln1}, we obtain
\begin{equation}
\label{eq:u^n)nl}
\begin{aligned}
    v_{nln}(t_i^+) &= |E_n|(\gamma-1)|\mathcal{C}_{bl}(n\omega)| \sin(i(n+1)\pi +\angle\mathcal{L}_{nl}(n\omega) \\
    &\ \ \ \ \ \ \ \ \ \ \ \ \  - \angle (1+\mathcal{L}_{bl}(n\omega)) +\angle \mathcal{C}_{bl}(n\omega)).
\end{aligned}   
\end{equation}
Let 
\begin{equation}
\label{eq:eta11}
\begin{aligned}
\eta_1(\omega) &= (\gamma-1)\lvert\mathcal{C}_{bl}(\omega)\rvert \sin(i\pi + \angle \mathcal{C}_{bl}(\omega)),\\
	\eta_n(\omega) &= (\gamma-1)|\mathcal{C}_{bl}(n\omega)| \sin(i(n+1)\pi +\angle\mathcal{L}_{nl}(n\omega) \\
  &\ \ \ \ \ \ \ \ \ - \angle (1+\mathcal{L}_{bl}(n\omega)) +\angle \mathcal{C}_{bl}(n\omega)).    
\end{aligned}
\end{equation}
Then, functions $v_{nl1}(t_i^+)$ in \eqref{eq:unl1_t} and $v_{nln}(t_i^+)$ in \eqref{eq:u^n)nl} are given by 
\begin{equation}
\label{eq:u_nln+}
\begin{aligned}
    v_{nl1}(t_i^+) = |E_1|\eta_1(\omega),\ \text{and }  v_{nln}(t_i^+) = |E_n|\eta_n(\omega).
\end{aligned}	
\end{equation}
Combining \eqref{eq: Gamma_defn} and \eqref{eq:u_nln+}, we obtain
\begin{equation}
\label{eq:G(w)1}
    \Gamma(\omega) = \frac{\sum\nolimits_{n=1}^{\infty}v_{nln}(t_i^+)}{v_{nl1}(t_i^+)} = \frac{\sum\nolimits_{n=1}^{\infty}|E_n| \eta_n(\omega)}{|E_1|\eta_1(\omega)}.
\end{equation}
Let
\begin{equation}
\label{eq:zeta}
	\zeta(n\omega) = \frac{|\mathcal{L}_{nl}(n\omega)|}{|1+\mathcal{L}_{bl}(n\omega)|},
\end{equation}
and substitute it to \eqref{eq: phase and Mag2}, we then have 
\begin{equation}
	\label{eq: Rn2}
	|E_n| = \Gamma(\omega)\zeta(n\omega)|E_1|.
\end{equation}
Substituting \eqref{eq: Rn2} to \eqref{eq:G(w)1}, $\Gamma(\omega)$ is derived as
	\begin{equation}
		\label{eq: gamma_final}		
		\begin{aligned}
		  \Gamma(\omega) &= 1/\left(1-\frac{\sum\nolimits_{n=3}^{\infty}\zeta(n\omega)\eta_n(\omega)}{\eta_1(\omega)}\right).
		\end{aligned}
	\end{equation}	
The value of $i\in \mathbb{Z}^+$ does not affect the result, regardless of its specific value. For simplicity, we choose $i=1$. Then, $\Gamma(\omega)$ in \eqref{eq: Gamma for PP-RCS} is derived. The n$^{\text{th}}$ sensitivity function $\mathcal{S}_n(n\omega)$ for closed-loop PP-RCSs is derived as the same as \cite{zhang2022frequency}.
\end{proof}
% \begin{cor}(Alt-open-loop transfer function for )
\begin{cor}(Steady-state Error Signal $e(t)$ in PP-RCSs)
Under Assumption \ref{assum: TwoReset}, applying the \enquote{Virtual Harmonics Generator}, the error signal $e(t)$ at steady-states in a SISO closed-loop PP-RCS with a sinusoidal reference signal $r(t) = R_0\sin(\omega t)$ is given by
    \begin{equation}
    \label{eq: y,e,u}
        \begin{aligned}
            e(t) &= \sum\nolimits_{n=1}^{\infty}\mathscr{F}^{-1}\left[\mathcal{S}_n(n\omega)R_n(n\omega)\right].
        \end{aligned}
    \end{equation}
    where $R_n(n\omega)$ is defined as
    \begin{equation}
        R_n(n\omega) = \mathscr{F}[r_n(t)] = \mathscr{F}[R_0\sin(n\omega t)].
    \end{equation}
\end{cor}

\subsection{Case Study 1: }
In this study, we have developed two Parallel-Partial Reset Control Systems (PP-RCSs) for a motion stage, represented as a MSD system in \eqref{eq:P(s)}. 

For validation, a one-degree precision motion stage (\cite{karbasizadeh2020band}) is utilised. Figure \ref{fig1: Bode2 of spider} presents the measured Frequency Response Function (FRF) data for this stage obtained from experiments. To streamline control system design, we identified the transfer function for the system using MATLAB's identification tool, denoted as $\mathcal{P}(s)$ in \eqref{eq:P(s)}. This transfer function represents a single eigenmode mass-spring-damper model.
\begin{equation}
\label{eq:P(s)}
    \mathcal{P}(s) = \frac{6.615e5}{83.57s^2+279.4s+5.837e5}.
\end{equation}
\subsection{Parallel-Partial-Reset Control Systems}

The structure of the PP-PCI-PID controller is illustrated in Fig. \ref{fig: 2_control system structures}(a). To address potential limit cycle issues associated with PCID in practical applications \cite{hosseinnia2013fractional}, an additional integrator has been incorporated. The integral parameter for the PP-PCI-PID controller is set to $\omega_i = 2\pi\cdot 15$ rad/s.
\begin{figure}[htp]
	\centering
	%	\missingfigure{CLCI}
	\includegraphics[width=0.9\columnwidth]{Figs/PCI_control system structure.pdf}
	\caption{(a)Parallel-Partial Proportional-Clegg-Integrator-PID (PP-PCI-PID) control system structure and (b) Parallel-Partial CgLp-PI$^2$D (PP-CgLp-PI$^2$D) control system structure, where $\omega_c = 2\pi\cdot 150$ rad/s.}
	\label{fig: 2_control system structures}
\end{figure}

The \enquote{Constant in Gain Lead in Phase} (CgLp) component serves to enhance phase lead without compromising gain advantages \cite{saikumar2019constant}. As for the PP-CgLp-PI$^2$D controller, its configuration is depicted in Fig. \ref{fig: 2_control system structures}(b).

The parameters in the PID (PI$^2$D) structure in both controllers are designed to achieve a bandwidth of 150 Hz and a phase margin of 50$\degree$ in open-loop, with varying combinations of the proportional gain value $k_{rc}$ and reset value $\gamma$ in Table \ref{tb: er}.
% \subsection{The Accuracy of the New Analysis Method}
Figure \ref{fig1: PCIID_n7_krcp5_PE_final} compares predictive accuracy between the closed-loop HOSIDF method (Theorem \ref{thm: Closed-loop HOSIDF for PP-RCS}) and the DF method, on the PP-PCI-PID system with arbitrarily chosen parameters $(\gamma,\ k_{rc}) = (-0.7,\ 0.5)$. Figure \ref{fig1: PCIID_50_150_er} visualises the error signal $e(t)$ for PP-PCI-PID under a sinusoidal reference input signal $r(t) = \sin (2\pi f t)$ when $f = 100$ Hz and $f = 1000$ Hz, obtained from simulations, the closed-loop HOSIDF based on equation \eqref{eq: y,e,u}, and the DF. Key conclusions are drawn:
\begin{figure}[htp]
	%	\missingfigure{RCsystem}
	\centerline{\includegraphics[width=0.9\columnwidth]{Figs/PCIID_n7_krcp5_et_final.pdf}}
	\caption{The error signal $e(t)$ of PP-PCI-PID with $(\gamma,\ k_{rc}) = (-0.7,\ 0.5)$ at input frequencies (a) $f = 100$ Hz and (b) $f = 1000$ Hz. Black lines are from simulation, blue and dashed lines are from closed-loop HOSIDF analysis in \eqref{eq: y,e,u}, and grey and dotted lines are from the DF analysis. Zoom-in details are depicted overlaid on the main figures.}
	\label{fig1: PCIID_50_150_er}
\end{figure}

\begin{enumerate}
    \item There is substantial improvement in accuracy achieved by the new HOSIDF method for analyzing closed-loop PP-PCI-PID systems, as evident in Fig. \ref{fig1: PCIID_n7_krcp5_PE_final}($a_2$), ($b_2$), ($a_3$), and ($b_3$), is noteworthy. This improvement, exceeding 100\% in some cases, is attributed to the fact that the DF method only considers the first-order harmonic in the calculation process (assuming $\Gamma(\omega)=0$ in \eqref{eq: gamma_final}), while reset systems inherently contain infinite harmonics. The increased precision of the new HOSIDF compared to the DF results from incorporating higher-order harmonics through the introduction of the parameter $\Gamma(\omega)$ into the analysis.
    \item As shown in Fig. \ref{fig1: PCIID_n7_krcp5_PE_final}($a_2$) and ($b_2$), the HOSIDF prediction error is larger at low frequencies compared to higher frequencies. This distinction arises from the HOSIDF method's foundational assumption of two resets per cycle, which holds true at high frequencies but does not accurately represent the behavior of multiple resets at lower frequencies in PP-PCI-PID systems \cite{zhang2023frequency}.
    \item The discrepancies between HOSIDF-predicted and simulated results arise from the fact that the HOSIDF method considers a finite number of harmonics, while practical systems involve an infinite number of harmonics.  In Fig. \ref{fig1: PCIID_n7_krcp5_RPE_final}(a), we illustrate the relationship between PE$_e$ (prediction error) at an input frequency of 1000 Hz and the number of harmonics ($N_h$) considered in the analysis. Increasing the number of harmonics in the calculation generally reduces prediction errors. However, a higher number of harmonics also leads to increased computational complexity. Consequently, a practical trade-off exists between the number of harmonics considered and prediction precision. In this particular case, a value of $N_h$ = 31 represents the optimal trade-off. While considering an infinite number of harmonics should theoretically result in zero error, in this figure, it converges to a very small constant value, which we attribute to the numerical error of the simulation. To further validate this, Figure \ref{fig1: PCIID_n7_krcp5_RPE_final}(b) was simulated with a larger step time. As seen, the same trend persists, but the error converges to an even smaller constant value.
\end{enumerate}
\begin{figure}[htp]
	%	\missingfigure{RCsystem}
	\centerline{\includegraphics[width=0.5\textwidth]{Figs/pp_pciid_PE_e_1000Hz_final.pdf}}
	\caption{The correlation between $\text{PE}_e$ at an input frequency of 1000 Hz and the number of harmonics, denoted as $N_h$, in the PP-PCI-PID system. Sub-figures (a) and (b) are results based on simulation results using different step time of 1e-7 and 1e-5, respectively.}
	\label{fig1: PCIID_n7_krcp5_RPE_final}
\end{figure}

==> 0_5_Results.tex <==
\section{Main Results}
\label{sec: result}
\subsection{Precision Positioning Setup}
For validation, a one-degree precision motion stage (\cite{karbasizadeh2020band}) is utilised. Figure \ref{fig1: Bode2 of spider} presents the measured Frequency Response Function (FRF) data for this stage obtained from experiments. To streamline control system design, we identified the transfer function for the system using MATLAB's identification tool, denoted as $\mathcal{P}(s)$ in \eqref{eq:P(s)}. This transfer function represents a single eigenmode mass-spring-damper model.
\begin{equation}
\label{eq:P(s)}
    \mathcal{P}(s) = \frac{6.615e5}{83.57s^2+279.4s+5.837e5}.
\end{equation}
% \begin{figure}[htp]
% 	%	\missingfigure{RCsystem}
% 	\centerline{\includegraphics[width=0.7\columnwidth]{Figs/Spider.pdf}}
% 	\caption{The planar precision positioning system with three degrees of freedom, denoted as \enquote{Spider}. It is driven by three voice coil actuators, labelled $A_1$, $A_2$, and $A_3$, with each actuator being directly linked to a corresponding mass, represented as $M_1$, $M_2$, and $M_3$. These masses are connected solely to the base, labelled as $M_C$, through dual leaf flexures. Sensing of the mass positions is facilitated by linear encoders denoted as \enquote{Enc}.}
% 	\label{fig1:spider}
% \end{figure}
% \begin{figure}[htp]
% 	%	\missingfigure{RCsystem}
% 	\centerline{\includegraphics[width=0.9\columnwidth]{Figs/Bode2_spider_hg.pdf}}
% 	\caption{FRF data of the precision motion stage.}
% 	\label{fig1: Bode2 of spider}
% \end{figure}
\subsection{Parallel-Partial-Reset Control Systems}
In this study, we have developed two Parallel-Partial Reset Control Systems (PP-RCSs) for a motion stage, represented as a MSD system in \eqref{eq:P(s)}. 

The structure of the PP-PCI-PID controller is illustrated in Fig. \ref{fig: 2_control system structures}(a). To address potential limit cycle issues associated with PCID in practical applications \cite{hosseinnia2013fractional}, an additional integrator has been incorporated. The integral parameter for the PP-PCI-PID controller is set to $\omega_i = 2\pi\cdot 15$ rad/s.
\begin{figure}[htp]
	\centering
	%	\missingfigure{CLCI}
	\includegraphics[width=0.9\columnwidth]{Figs/PCI_control system structure.pdf}
	\caption{(a)Parallel-Partial Proportional-Clegg-Integrator-PID (PP-PCI-PID) control system structure and (b) Parallel-Partial CgLp-PI$^2$D (PP-CgLp-PI$^2$D) control system structure, where $\omega_c = 2\pi\cdot 150$ rad/s.}
	\label{fig: 2_control system structures}
\end{figure}

The \enquote{Constant in Gain Lead in Phase} (CgLp) component serves to enhance phase lead without compromising gain advantages \cite{saikumar2019constant}. As for the PP-CgLp-PI$^2$D controller, its configuration is depicted in Fig. \ref{fig: 2_control system structures}(b).
% \begin{figure}[htp]
% 	\centering
% 	%	\missingfigure{CLCI}
% 	\includegraphics[width=0.98\columnwidth]{Figs/CgLp_control system structure.pdf}
% 	\caption{Parallel-Partial CgLp-PI$^2$D (PP-CgLp-PI$^2$D) control system structure, where $\omega_c = 2\pi\cdot 150$ rad/s. }
% 	\label{fig: CgLp control system structure}
% \end{figure}

The parameters in the PID (PI$^2$D) structure in both controllers are designed to achieve a bandwidth of 150 Hz and a phase margin of 50$\degree$ in open-loop, with varying combinations of the proportional gain value $k_{rc}$ and reset value $\gamma$ in Table \ref{tb: er}.
\subsection{The Accuracy of the New Analysis Method}
Figure \ref{fig1: PCIID_n7_krcp5_PE_final} compares predictive accuracy between the closed-loop HOSIDF method (Theorem \ref{thm: Closed-loop HOSIDF for PP-RCS}) and the DF method, on the PP-PCI-PID system with arbitrarily chosen parameters $(\gamma,\ k_{rc}) = (-0.7,\ 0.5)$. Figure \ref{fig1: PCIID_50_150_er} visualises the error signal $e(t)$ for PP-PCI-PID under a sinusoidal reference input signal $r(t) = \sin (2\pi f t)$ when $f = 100$ Hz and $f = 1000$ Hz, obtained from simulations, the closed-loop HOSIDF based on equation \eqref{eq: y,e,u}, and the DF. Key conclusions are drawn:
\begin{figure}[htp]
	%	\missingfigure{RCsystem}
	\centerline{\includegraphics[width=0.9\columnwidth]{Figs/PCIID_n7_krcp5_et_final.pdf}}
	\caption{The error signal $e(t)$ of PP-PCI-PID with $(\gamma,\ k_{rc}) = (-0.7,\ 0.5)$ at input frequencies (a) $f = 100$ Hz and (b) $f = 1000$ Hz. Black lines are from simulation, blue and dashed lines are from closed-loop HOSIDF analysis in \eqref{eq: y,e,u}, and grey and dotted lines are from the DF analysis. Zoom-in details are depicted overlaid on the main figures.}
	\label{fig1: PCIID_50_150_er}
\end{figure}
\begin{defn}
The Root Mean Square (RMS) values of the error signal $e(t)$ from Simulink, the new closed-loop HOSIDF, and the DF are denoted as $||e||_2^{sim}$, $||e||_2^{HOSIDF}$, and $||e||_2^{DF}$, respectively. Similarly, the RMS values of the control input signal $u(t)$ are represented as $||u||_2^{sim}$, $||u||_2^{HOSIDF}$, and $||u||_2^{DF}$. 

The Prediction Error (PE) PE$_e$ and PE$_u$ are the absolute differences between the RMS values of $e(t)$ and $u(t)$ obtained from simulation and frequency-domain analysis methods, respectively.
\begin{equation}
    \begin{aligned}
      \text{PE}_e = {\bigg| ||e||_2^{sim} -||e||_2^{Model}\bigg|},\ \   \text{PE}_u = {\bigg| ||u||_2^{sim}-||u||_2^{Model} \bigg|}.
    \end{aligned}
\end{equation}  
The precision advancement (PA) of the HOSIDF compared to the DF is defined as 
\begin{equation}
    \begin{aligned}
      \text{PA}_e = \frac{\bigg|  \text{PE}_e^{DF} - \text{PE}_e^{HOSIDF} \bigg|}{||e||_2^{sim}},\  \text{PA}_u = \frac{\bigg|  \text{PE}_u^{DF} - \text{PE}_u^{HOSIDF} \bigg|}{||u||_2^{sim}}.
    \end{aligned}
\end{equation}
\end{defn}   
% The Relative Prediction Error (RPE) of the error signal $e(t)$ is defined as 
% \begin{equation}
%     \begin{aligned}
%       \text{RPE}_e (\%) = \frac{\text{PE}_e}{||e||_2^{sim}}\cdot 100\%.
%     \end{aligned}
% \end{equation} 

\begin{figure}[htp]
	%	\missingfigure{RCsystem}
	\centerline{\includegraphics[width=0.45\textwidth]{Figs/PCIID_n7_krcp5_PE_final.pdf}}
	\caption{($a_1$) The RMS, ($a_2$) the PE, and ($a_3$) the PA of error signal $e(t)$ of the PP-PCI-PID system with parameters $(\gamma,\ k_{rc}) = (-0.7,\ 0.5)$. ($b_1$) The RMS, ($b_2$) the PE, and ($b_3$) the PA of control input signal $u(t)$.}
	\label{fig1: PCIID_n7_krcp5_PE_final}
\end{figure}

\begin{enumerate}
    \item There is substantial improvement in accuracy achieved by the new HOSIDF method for analyzing closed-loop PP-PCI-PID systems, as evident in Fig. \ref{fig1: PCIID_n7_krcp5_PE_final}($a_2$), ($b_2$), ($a_3$), and ($b_3$), is noteworthy. This improvement, exceeding 100\% in some cases, is attributed to the fact that the DF method only considers the first-order harmonic in the calculation process (assuming $\Gamma(\omega)=0$ in \eqref{eq: gamma_final}), while reset systems inherently contain infinite harmonics. The increased precision of the new HOSIDF compared to the DF results from incorporating higher-order harmonics through the introduction of the parameter $\Gamma(\omega)$ into the analysis.
    \item As shown in Fig. \ref{fig1: PCIID_n7_krcp5_PE_final}($a_2$) and ($b_2$), the HOSIDF prediction error is larger at low frequencies compared to higher frequencies. This distinction arises from the HOSIDF method's foundational assumption of two resets per cycle, which holds true at high frequencies but does not accurately represent the behavior of multiple resets at lower frequencies in PP-PCI-PID systems \cite{zhang2023frequency}.
    \item The discrepancies between HOSIDF-predicted and simulated results arise from the fact that the HOSIDF method considers a finite number of harmonics, while practical systems involve an infinite number of harmonics.  In Fig. \ref{fig1: PCIID_n7_krcp5_RPE_final}(a), we illustrate the relationship between PE$_e$ (prediction error) at an input frequency of 1000 Hz and the number of harmonics ($N_h$) considered in the analysis. Increasing the number of harmonics in the calculation generally reduces prediction errors. However, a higher number of harmonics also leads to increased computational complexity. Consequently, a practical trade-off exists between the number of harmonics considered and prediction precision. In this particular case, a value of $N_h$ = 31 represents the optimal trade-off. While considering an infinite number of harmonics should theoretically result in zero error, in this figure, it converges to a very small constant value, which we attribute to the numerical error of the simulation. To further validate this, Figure \ref{fig1: PCIID_n7_krcp5_RPE_final}(b) was simulated with a larger step time. As seen, the same trend persists, but the error converges to an even smaller constant value.
    % between (a) the RMS of the RPE ($||\text{RPE}_e||_2$) across the entire frequency spectrum, (b) the RPE at an input frequency of 1000 Hz, and (c) the RPE at an input frequency of 10 Hz, with respect to the number of harmonics ($N_h$) considered in the analysis. Increasing the number of harmonics in the calculation tends to reduce relative prediction errors across the entire frequency spectrum. The prediction precision is more substantial at high frequency (1000 Hz) compared to low frequency (10 Hz) due to the two-reset assumption not holding at low frequencies. However, a higher number of harmonics also leads to increased computational complexity. Therefore, there's a practical trade-off between the number of harmonics considered and prediction precision. In this case, $N_h=31$ was chosen.
\end{enumerate}
\begin{figure}[htp]
	%	\missingfigure{RCsystem}
	\centerline{\includegraphics[width=0.5\textwidth]{Figs/PCIID_n7_krcp5_PE_1000Hz_final.pdf}}
	\caption{The correlation between $\text{PE}_e$ at an input frequency of 1000 Hz and the number of harmonics, denoted as $N_h$, in the PP-PCI-PID system. Sub-figures (a) and (b) are results based on simulation results using different step time of 1e-7 and 1e-5, respectively.}
	\label{fig1: PCIID_n7_krcp5_RPE_final}
\end{figure}
% \begin{figure}[htp]
% 	%	\missingfigure{RCsystem}
% 	\centerline{\includegraphics[width=0.5\textwidth]{Figs/PCIID_n7_krcp5_RPE_final.pdf}}
% 	\caption{The correlation between (a) $||\text{RPE}_e||_2$, (b) $\text{RPE}_e$ at an input frequency of 1000 Hz, and (c) $\text{RPE}_e$ at an input frequency of 10 Hz, and the number of harmonics, denoted as $N_h$, in the PP-PCI-PID system.}
% 	\label{fig1: PCIID_n7_krcp5_RPE_final}
% \end{figure}
\subsection{The Application of the Closed-loop HOSIDF for The Design of PP-RCSs}
% \begin{defn}
% The Cumulative Power Spectral Density (CPSD) of the error signal obtained from \eqref{eq: y,e,u} at 1000 Hz defined as CPDS$_e$ is employed as a metric to assess steady-state error.    
% \end{defn}
\begin{figure}[htp]
	\centering
	%	\missingfigure{CLCI}
	\includegraphics[width=0.95\columnwidth]{Figs/CgLp_control system structure.pdf}
	\caption{(a)Parallel-Partial Proportional-Clegg-Integrator-PID (PP-PCI-PID) control system structure and (b) Parallel-Partial CgLp-PI$^2$D (PP-CgLp-PI$^2$D) control system structure, where $\omega_c = 2\pi\cdot 150$ rad/s.}
	\label{fig: 2_control system structures}
\end{figure}
We have configured 7 PP-PCI-PID and 7 PP-CgLp-PI$^2$D control systems under sinusoidal input $r(t) = \sin(2\pi f t)$ with varying $(\gamma, k_{rc})$ values, as detailed in Table \ref{tb: er}. These systems, however, share a common set of open-loop specifications: a bandwidth of 150 Hz and a phase margin of 50$\degree$, as demonstrated in Fig. \ref{fig1:PP_PCIID_Results}(a) and Fig. \ref{fig1:PP_CgLp_results}(a). The predicted closed-loop $||e||_2^{HOSIDF}$ and $||e||_\infty^{HOSIDF}$(the maximum value of steady-state errors) values, are presented in Fig. \ref{fig1:PP_PCIID_Results}(b) and Fig. \ref{fig1:PP_CgLp_results}(b), calculated using Theorem \ref{thm: Closed-loop HOSIDF for PP-RCS} and including 31 harmonics.
\begin{table}[htp]
\caption{The predicted $||e||_2^{HOSIDF}$ values for 7 PP-PCI-PID and \textcolor{blue}{PP-CgLp-PI$^2$D} control systems under inputs with frequencies of 10 Hz, 100 Hz, and 500 Hz.}
\label{tb: er}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{RCs}  & \multirow{2}{*}{Cases}  & \multirow{2}{*}{($\gamma$, $k_{rc}$)} & \multicolumn{6}{c|}{$||e||_2^{HOSIDF}$(dB)}\\ \cline{4-9} 
& & & \multicolumn{2}{c|}{10 Hz} & \multicolumn{2}{c|}{100 Hz} & \multicolumn{2}{c|}{500 Hz}\\ \hline
 & $C_1$& (-0.5,1.0)  & -48.61 & \textcolor{blue}{-54.74} & -5.56 & \textcolor{blue}{-2.64} & -1.52 & \textcolor{blue}{-2.03} \\ \cline{2-9} 
 & $C_2$& (0.0,1.0)  & -50.18  & \textcolor{blue}{-53.49} &  -4.70 & \textcolor{blue}{-3.20} & -1.30 & \textcolor{blue}{-1.80} \\ \cline{2-9} 
\multirow{2}{*}{PP-PCI-PID} & $C_3$& (0.4,1.0)  & -50.09  & \textcolor{blue}{-52.01} & -4.37  & \textcolor{blue}{-3.62} & -1.23  & \textcolor{blue}{-1.55} \\ \cline{2-9}  
\multirow{2}{*}{\textcolor{blue}{PP-CgLp-PI$^2$D}} & $C_4$& (0.0,0.7)  & -50.24  & \textcolor{blue}{-52.46} & -4.53  & \textcolor{blue}{-3.50} & -1.27  & \textcolor{blue}{-1.67} \\ \cline{2-9} 
 & $C_5$& (-0.8,0.7) & -46.01 & \textcolor{blue}{-54.28} & -6.42  & \textcolor{blue}{-2.84} & -1.76  & \textcolor{blue}{-2.08} \\ \cline{2-9} 
 & $C_6$& (0.7,0.7)  & -49.46  & \textcolor{blue}{-50.08} & -4.17  & \textcolor{blue}{-3.96} & -1.18  &  \textcolor{blue}{-1.28}\\  \cline{2-9} 
 & $C_7$& (1.0,1.0)  & -49.00  & \textcolor{blue}{-48.79} & -4.08  & \textcolor{blue}{-4.11} & -1.16  &  \textcolor{blue}{-1.16}\\ \hline
\end{tabular}
}
\end{table}
% \begin{figure}[htp]
% 	%	\missingfigure{RCsystem}
% 	\centerline{\includegraphics[width=1\columnwidth]{Figs/PP_PCIID_Lo.pdf}}
% 	\caption{The open-loop bode plots of 7 PP-PCI-PID control systems (($C_1$-$C_7$ in Table \ref{tb: er})).}
% 	\label{fig1:PP_PCIID_Lo}
% \end{figure}
% \begin{figure}[htp]
% 	%	\missingfigure{RCsystem}
% 	\centerline{\includegraphics[width=1\columnwidth]{Figs/PP_CgLp_Lo.pdf}}
% 	\caption{The open-loop bode plots of 7 PP-CgLp-PI$^2$D control systems (($C_1$-$C_7$ in Table \ref{tb: er})).}
% 	\label{fig1:PP_CgLp_Lo}
% \end{figure}
\begin{figure}[htp]
	%	\missingfigure{RCsystem}
	\centerline{\includegraphics[width=1\columnwidth]{Figs/PP_PCIID_Results.pdf}}
	\caption{(a) The open-loop Bode plots, (b) $||e||_2^{HOSIDF}$, and (c) $||e||_\infty^{HOSIDF}$ of 7 PP-PCI-PID control systems (denoted as $C_1-C_7$), as predicted by Theorem \ref{thm: Closed-loop HOSIDF for PP-RCS}. Detailed validation in Table \ref{tb: er} is conducted at three selected frequencies, indicated by red dashed lines. (d) Simulated steady-state errors of $C_1-C_7$ at an input frequency of 10 Hz.}
	\label{fig1:PP_PCIID_Results}
\end{figure}
\begin{figure}[htp]
	%	\missingfigure{RCsystem}
	\centerline{\includegraphics[width=0.95\columnwidth]{Figs/PP_CgLp_results.pdf}}
	\caption{(a) The open-loop Bode plots, (b) $||e||_2^{HOSIDF}$, and (c) $||e||_\infty^{HOSIDF}$ of 7 PP-CgLp-PI$^2$D control systems (designated as $C_1-C_7$), as predicted by Theorem \ref{thm: Closed-loop HOSIDF for PP-RCS}. (d) Simulated steady-state errors of $C_1-C_7$ at an input frequency of 10 Hz.}
	\label{fig1:PP_CgLp_results}
\end{figure}

We perform simulations at low-frequency (10 Hz), mid-frequency (100 Hz), and high-frequency (500 Hz). 
% Their RMS values of steady-state errors $||e||_2^{sim}$ are denoted by scattered points on Fig. \ref{fig1:pp_pciid_er_model_sim} and Fig. \ref{fig1:pp_cglp_er_model_sim}. 
The predicted $||e||_2^{HOSIDF}$ values for the 14 cases at these three input frequencies are listed in Table \ref{tb: er}. The prediction errors between the predicted and simulated values (denoted as PE$_e\text{ (dB)}$ = $||e||_2^{HOSIDF}\text{ (dB)} -||e||_2^{sim}\text{ (dB)}$) are detailed in Table \ref{tb: PE}. 
\begin{table}[htp]
\caption{The PE$_e$ values for the 7 PP-PCI-PID and \textcolor{blue}{PP-CgLp-PI$^2$D} control systems under input frequencies of 10 Hz, 100 Hz, and 500 Hz.}
\label{tb: PE}
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{RCs}  & \multirow{2}{*}{Cases}  & \multirow{2}{*}{($\gamma$, $k_{rc}$)} & \multicolumn{6}{c|}{PE$_e$(dB)}\\ \cline{4-9} 
& & & \multicolumn{2}{c|}{10 Hz} & \multicolumn{2}{c|}{100 Hz} & \multicolumn{2}{c|}{500 Hz}\\ \hline
 & $C_1$& (-0.5,1.0)  & 0.64  & \textcolor{blue}{1.14e-3} & 0.14  & \textcolor{blue}{0.08} & 2.68e-3  & \textcolor{blue}{0.07} \\ \cline{2-9} 
 & $C_2$& (0.0,1.0)  & 0.71  & \textcolor{blue}{1.16e-4} & 0.03  & \textcolor{blue}{0.01} & 0  & \textcolor{blue}{0} \\ \cline{2-9} 
\multirow{2}{*}{PP-PCI-PID} & $C_3$& (0.4,1.0)  & 0.39  & \textcolor{blue}{3.95e-5} & 7.50e-3  & \textcolor{blue}{0.01} & 3.05e-3 & \textcolor{blue}{0.02} \\ \cline{2-9}  
\multirow{2}{*}{\textcolor{blue}{PP-CgLp-PI$^2$D}} & $C_4$& (0.0,0.7)  & 0.65 & \textcolor{blue}{4.28e-4} & 0.02 & \textcolor{blue}{0.01} & 2.87e-3 & \textcolor{blue}{0.03} \\ \cline{2-9} 
 & $C_5$& (-0.8,0.7) & 2.00  & \textcolor{blue}{6.39e-4} & 0.27  & \textcolor{blue}{0.03} & 5.07e-3  & \textcolor{blue}{0.08} \\ \cline{2-9} 
 & $C_6$& (0.7,0.7)  & 1.26  & \textcolor{blue}{2.88e-6} & 6.43e-4  & \textcolor{blue}{2.33e-3} & 2.80e-3  &  \textcolor{blue}{0.01}\\  \cline{2-9} 
 & $C_7$& (1.0,1.0)  & 2.74e-4  & \textcolor{blue}{1.32e-6} & 6.94e-5  & \textcolor{blue}{2.84e-4} & 2.37e-3  &  \textcolor{blue}{0.02}\\ \hline
\end{tabular}
}
\end{table}

The results in Table \ref{tb: PE} indicate that, in general, the prediction errors are small. However, at 10 Hz, the prediction errors in PP-PCI-PID systems are relatively larger. This discrepancy arises because the prediction method assumes the presence of two resets per steady-state cycle. Nevertheless, at low frequencies, PP-PCI-PID systems exhibit multiple resets, as illustrated in Fig. \ref{fig1:PP_PCIID_Results}(c). In contrast, the prediction errors in PP-CgLp-PI$^2$D systems remain small, as they consistently demonstrate two resets at low frequencies, as demonstrated in Fig. \ref{fig1:PP_CgLp_results}(c).
% \begin{figure}[htp]
% 	%	\missingfigure{RCsystem}
% 	\centerline{\includegraphics[width=1.1\columnwidth]{Figs/pp_pciid_sim_10Hz.pdf}}
% 	\caption{Simulated steady-state error of 7 PP-PCI-PID control systems at input frequency of 10 Hz.}
% 	\label{fig1:pp_pciid_sim_10Hz}
% \end{figure}
% \begin{figure}[htp]
% 	%	\missingfigure{RCsystem}
% 	\centerline{\includegraphics[width=1.1\columnwidth]{Figs/PP_CgLp_sim_10Hz.pdf}}
% 	\caption{Simulated steady-state error of 7 PP-CgLp-PI$^2$D control systems at input frequency of 10 Hz.}
% 	\label{fig1:PP_CgLp_sim_10Hz}
% \end{figure}

Based on the closed-loop analysis for PP-PCI-PID and PP-CgLp-PI$^2$D in Table \ref{tb: er}, the following conclusions can be drawn:
\begin{enumerate}
\item In both PP-PCI-PCID and PP-CgLp-PCID structures, cases $C_1$, $C_7$, and $C_5$ display the lowest RMS steady-state error in the low-frequency range (around (0-80) Hz), the mid-frequency range (around (80-120) Hz), and the high-frequency range (around (120-1000) Hz), respectively.
\item Despite both PP-PCI-PID and PP-CgLp-PI$^2$D systems having the same bandwidth and phase margin in open-loop, there are distinct performance differences: At low frequencies and high frequencies, the PP-CgLp-PI$^2$D structures deliver superior steady-state tracking precision. In contrast, at mid-frequency range, the PP-PCI-PID systems outperform in terms of tracking precision.
% It's worth noting that while the PCI-PID structure effectively prevents limit-cycle occurrences in the time domain compared to the PCID structure, 
Note that PP-PCI-PID introduces multiple-reset actions at lower frequencies. This results in larger error signal amplitudes, as demonstrated in Fig. \ref{fig1:PP_PCIID_Results}(c), and leads to analytical deviations as shown in Table \ref{tb: PE}. In contrast, PP-CgLp-PI$^2$D systems avoid multiple-reset at low frequencies, and they can be efficiently tuned using the method outlined in Theorem \ref{thm: Closed-loop HOSIDF for PP-RCS}.
\end{enumerate}

These results demonstrate that the new closed-loop HOSIDF approach is a valuable tool for designing PP-RCSs that achieve improved steady-state precision within specific frequency ranges. 
% \begin{figure}[htp]
% 	%	\missingfigure{RCsystem}
% 	\centerline{\includegraphics[width=0.9\columnwidth]{Figs/PP_PCIID_et_sum.pdf}}
% 	\caption{Simulated steady-state error signals for the 7 PP-PCI-PID control systems under single sinusoidal inputs with frequencies of (a) 5 Hz, (b) 80 Hz, and (c) 500 Hz.}
% 	\label{fig1: PP_PCIID_et_sum}
% \end{figure}
% \subsection{Applying the Analysis Method to Design PP-CgLp-PI$^2$D}
% \begin{table}[htp]
% \caption{The Prediction Error (PE) of the error signals $e(t)$ for 7 PP-CgLp-PI$^2$D control systems at input frequencies of 10 Hz, 100 Hz, and 500 Hz.}
% \label{tb: CgLp_piid}
% \centering
% \resizebox{0.85\columnwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{RC}  & \multirow{2}{*}{Cases}  & \multirow{2}{*}{($\gamma$, $k_{rc}$)} & \multicolumn{3}{c|}{PE$_e$(dB)}\\ \cline{4-6} 
% \multirow{8}{*}{PP-CgLp-PI$^2$D} & & & 10 Hz & 100 Hz & 500 Hz\\ \hline
%  & $C_1$& (-0.5,1.0) & & & \\ \cline{2-6} 
%  & $C_2$& (0.0,1.0)  & & & \\ \cline{2-6} 
%  & $C_3$& (0.4,1.0)  & & & \\ \cline{2-6}  
%  & $C_4$& (0.0,0.7)  & & & \\ \cline{2-6} 
%  & $C_5$& (-0.8,0.7)  & & & \\ \cline{2-6} 
%  & $C_6$& (0.7,0.7)  & & & \\  \cline{2-6} 
%  & $C_7$& (1.0,1.0)  & & & \\ \hline
% \end{tabular}
% }
% \end{table}
% \begin{figure}[htp]
% 	%	\missingfigure{RCsystem}
% 	\centerline{\includegraphics[width=0.95\columnwidth]{Figs/PP_CgLp_PIID_CPSD_final.pdf}}
% 	\caption{CPSD$_e$ of the 7 PP-CgLp-PI$^2$D cases $C_1-C_7$ predicted by Theorem \ref{thm: Closed-loop HOSIDF for PP-RCS}. Results at three input frequencies of 10 Hz, 100 Hz, and 500 Hz (in red circles) were applied to compared to simulated results in Fig. \ref{fig1: PP_CgLp_piid_et_sum}.}
% 	\label{fig1: PP_CgLp_piid_CPSD_FINAL}
% \end{figure}
% \begin{figure}[htp]
% 	%	\missingfigure{RCsystem}
% 	\centerline{\includegraphics[width=0.9\columnwidth]{Figs/PP_CgLp_PIID_et.pdf}}
% 	\caption{Simulated error signals for the 7 PP-CgLp-PI$^2$D control systems under single sinusoidal inputs with frequencies of (a) 10 Hz, (b) 100 Hz, and (c) 500 Hz.}
% 	\label{fig1: PP_CgLp_piid_et_sum}
% \end{figure}
% \subsection{The Influence of White Noise to The PP-RCSs}
% Figure \ref{fig1: PP_PCIID_et_nt}(a)-(c) display the steady-state error signals for three cases ($C_1$, $C_5$, and $C_7$) within PP-PCI-PID under the influence of white noise input signal $n(t)$ (shown with grey lines in Fig. \ref{fig1: PP_PCIID_et_nt}) and sinusoidal reference input $r(t) = \sin (10\pi t)$ at input frequencies of 5 Hz, 80 Hz, and 500 Hz, respectively. The outcomes indicate that the inclusion of noise does not significantly alter the relative performance of these three configurations observed in Fig. \ref{fig1: PP_PCIID_et_sum}. 

% The steady-state errors for three cases ($C_1$, $C_5$, and $C_7$) in PP-CgLp-PI$^2$D control systems under sinusoidal reference input $r(t) = \sin (2\pi f t)$ (f = 10, 100, 500 Hz) and noise input signal $n(t)$ are shown in Fig. \ref{fig1: PP_CgLp_PIID_et_nt}. These results are in alignment with the predictions shown in Fig. \ref{fig1: PP_CgLp_piid_CPSD_FINAL}. 
% \begin{figure}[htp]
% 	%	\missingfigure{RCsystem}
% 	\centerline{\includegraphics[width=\columnwidth]{Figs/PP_PCIID_et_nt.pdf}}
% 	\caption{The steady-state errors of the three cases $C_1$, $C_5$, and $C_7$ in PP-PCI-PID control systems under white noise inputs $n(t)$ (in grey) and reference inputs $r(t)$ at frequencies of 5 Hz, 80 Hz, and 500 Hz.}
% 	\label{fig1: PP_PCIID_et_nt}
% \end{figure}
% \begin{figure}[htp]
% 	%	\missingfigure{RCsystem}
% 	\centerline{\includegraphics[width=\columnwidth]{Figs/PP_CgLp_PIID_et_nt.pdf}}
% 	\caption{The steady-state errors of the three cases $C_1$, $C_5$, and $C_7$ in PP-CgLp-PI$^2$D control systems under white noise inputs $n(t)$ (in grey) and reference inputs $r(t)$ at frequencies of 10 Hz, 100 Hz, and 500 Hz.}
% 	\label{fig1: PP_CgLp_PIID_et_nt}
% \end{figure}
% The limited impact of noise can be attributed to the relatively low amplitudes of the introduced noise. Future research efforts should focus on in-depth investigations to enhance robustness against noise-induced effects on steady-state errors and include experimental validation.


==> Append.tex <==
\begin{rem}
For a RCS with higher-order (more than second-order) plants, before applying Theorem \ref{thm: Delta} to identify the presence of multiple-reset scenarios, a reduction to second-order systems based on the dominant pole approximation method (as outlined in \cite{rommes2008modal}) is required. Further calculations and validation through practical experimentation will be done in the future.
\end{rem}

Figure \ref{fig:case4} shows the error signal $e(t)$ and base-linear error signal $e_{bl}(t)$ of a RCS to illustrate Remark \ref{rem: ebl_mrcs}. The system employs a Proportional Clegg Integrator controller (\cite{hosseinnia2013fractional}) with a base-linear transfer function of $\frac{57120}{s}+628.32$ and a plant with transfer function $\frac{1}{0.009s^2+s}$. The input signal is a sinusoidal reference input $r(t)=\sin (2\pi f t)$ with $f=20$ Hz. The results indicate the presence of four zero-crossings in $e_{bl}(t)$ during the first transient cycle, resulting in multiple-reset in the RCS.
     \begin{figure}[H]
	%	\missingfigure{RCsystem}
	\centerline{\includegraphics[width=\columnwidth]{figs/bad_design.pdf}}
	\caption{The input signal $r(t)$ (in black, solid), the error signal $e(t)$ (in red, solid), and the base-linear error signal $e_{bl}(t)$ (in black, dashed) of a reset control system. The green circles are utilised to indicate the zero-crossing points of $e_{bl}(t)$, while the blue circles are used to mark the reset instants of the RCS in one period.}
	\label{fig:case4}
    \end{figure}




 Triangle wave reference tracking is commonly used in servo systems and motion control applications. Servo systems are used to control the position, speed, or acceleration of mechanical systems such as robotic arms, CNC machines, or motor drives. When using a triangular wave as the reference input, the control system's response is observed as it attempts to track the changing reference signal. The system's ability to follow the rapidly changing input and its responsiveness to the varying slopes of the triangular wave can reveal valuable insights into the system's dynamic behavioUr and tracking performance. By applying a triangular wave as the reference input, engineers can test how well the servo system tracks the varying set-points and handles dynamic motion profiles.

==> appen.tex <==
\section{True first reset instant}

\subsubsection{Model for multiple reset systems}
\begin{rem}
	Suppose $p_i, \ i \in \mathbb{N}^k$ is the pole of $\mathcal{S}_{bl}(\omega)$, with $k$ being the number of the poles. Similarly, $q_i, \ i \in \mathbb{N}^m$ is defined as the pole of $\mathcal{T}_{bl}(\omega)$, with $m$ being the number of its poles. Then $\mathcal{S}_{bl}(\omega)$ and $\mathcal{T}_{bl}(\omega)$ can be represented by
	\begin{equation}
		\label{eq: Sbl1,Tbl1}
		\begin{aligned}
			\mathcal{S}_{bl}(\omega) &= {S}_{bl}(\omega)\prod_{i=1}^{i=k}\frac{j\omega-p_i}{j\omega-p_i},\\
			\mathcal{T}_{bl}(\omega) &= {T}_{bl}(\omega)\prod_{i=1}^{i=m}\frac{j\omega-q_i}{j\omega-q_i},
		\end{aligned}
	\end{equation}
	where $\omega$ is an arbitrary angular frequency.
\end{rem}
\begin{lem}
	In time-domain, the transient and steady-state responses of error $e_{bl}(t)$ and output $y_{bl}(t)$ of base-linear $\mathcal{RCS}$ in closed-loop with respect to the a sinusoidal input signal $r(t) = A\sin (\omega t)$ whose Fourier transform is $R(\omega) = \mathscr{F}[r(t)]$ are given by
	\begin{equation}
		\label{eq: ebl}
		\begin{aligned}
			e_{bl}(t) &= e_{blss}(t) + e_{blts}(t),\\
			e_{blss}(t) &= A|\mathcal{S}_{bl}(\omega)|\sin \left[ \omega t+ \angle \mathcal{S}_{bl}(\omega)\right] ,\\
			e_{blts}(t) &= - A|\mathcal{S}_{bl}(\omega)|\sum_{i=1}^{i=k}e^{p_i t} \sin \left( \angle \mathcal{S}_{bl}(\omega)\right),
		\end{aligned}
	\end{equation}
and
	\begin{equation}
		\label{eq: ybl}
		\begin{aligned}
			y_{bl}(t) &= y_{blss}(t) + y_{blts}(t),\\
			y_{blss}(t) &= A|\mathcal{T}_{bl}(\omega)|\sin \left[ \omega t+ \angle \mathcal{T}_{bl}(\omega)\right] ,\\
			y_{blts}(t) &= -A|\mathcal{T}_{bl}(\omega)| \sum_{i=1}^{i=m}e^{q_i t} \sin \left( \angle \mathcal{T}_{bl}(\omega)\right),
		\end{aligned}
	\end{equation}
where $e_{blss}(t)$ and $y_{blss}(t)$, $e_{blts}(t)$ and $y_{blts}(t)$ are the steady-state responses and transient-state responses of $e_{bl}(t)$ and $y_{bl}(t)$ respectively.
\end{lem}

\begin{pf}
	For an exponential input signal $r_e(t) = e^{j\omega t}$ whose Fourier transform is $R_e(\omega) = \mathscr{F}[r_e(t)]=\frac{1}{j\omega-j\omega}$, the error $E_{bl}(\omega)$ and output $Y_{bl}(\omega)$ of base-linear $\mathcal{RCS}$ are given by
	\begin{equation}
		\begin{aligned}
			E_{bl}(\omega) &= R_e(\omega)S_{bl}(\omega) &= \frac{S_{bl}(\omega)}{j\omega-j\omega},\\
			Y_{bl}(\omega) &= R_e(\omega)T_{bl}(\omega) &= \frac{T_{bl}(\omega)}{j\omega-j\omega}.	
		\end{aligned}
	\end{equation}
	
	From \eqref{eq: Sbl1,Tbl1}, $E_{bl}(\omega)$ and $Y_{bl}(\omega)$ can be given by
	\begin{equation}
		\begin{aligned}
			E_{bl}(\omega) &= \frac{\mathcal{S}_{bl}(\omega)}{j\omega-j\omega} - \sum_{i=1}^{i=k}\frac{\mathcal{S}_{bl}(\omega)}{j\omega-p_i},\\
			Y_{bl}(j\omega) &= \frac{\mathcal{T}_{bl}(\omega)}{j\omega-j\omega} - \sum_{i=1}^{i=m}\frac{\mathcal{T}_{bl}(\omega)}{j\omega-q_i}.
		\end{aligned}
	\end{equation}
	
	$e_{blss}(t)$ and $e_{blts}(t)$ are the steady-state response and transient-state response of $e_{bl}(t)$ which are given by
	\begin{equation}
		\begin{aligned}
			e_{bl}(t) &= e_{blss}(t) + e_{blts}(t),\\
			e_{blss}(t) &= \mathscr{F}^{-1}\left[ \frac{\mathcal{S}_{bl}(\omega)}{j\omega-j\omega}\right]  = e^{j\left[ \omega t+\mathcal{S}_{bl}(\omega)\right] } ,\\
			e_{blts}(t) &= \mathscr{F}^{-1}\left[ - \sum_{i=1}^{i=k}\frac{\mathcal{S}_{bl}(\omega)}{j\omega-p_i}\right] = -\sum_{i=1}^{i=k}e^{p_i t} e^{j\mathcal{S}_{bl}(\omega)}.
		\end{aligned}
	\end{equation}

	Based on the \enquote{\emph{Euler Formula}}, for a sinusoidal input signal $r(t) = A\sin (\omega t)$ whose Fourier transform is $R(\omega) = \mathscr{F}[r(t)]$, the steady-state response $e_{blss}(t)$ and transient-state response $e_{blts}(t)$ of error signal $e_{bl}(t)$ are given by
	\begin{equation}
	\label{eq: ebl}
		\begin{aligned}
			e_{bl}(t) &= e_{blss}(t) + e_{blts}(t),\\
			e_{blss}(t) &= A|\mathcal{S}_{bl}(\omega)|\sin \left[ \omega t+ \angle \mathcal{S}_{bl}(\omega)\right] ,\\
			e_{blts}(t) &= - A|\mathcal{S}_{bl}(\omega)|\sum_{i=1}^{i=k}e^{p_i t} \sin \left( \angle \mathcal{S}_{bl}(\omega)\right).
		\end{aligned}
	\end{equation}
	
	The steady-state response $y_{blss}(t)$ and transient-state response $y_{blts}(t)$ of output signal $y_{bl}(t)$ in \eqref{eq: ybl} can be derived as the same process as above.
\end{pf}

\begin{lem}
	For a sinusoidal input signal $r(t) = A\sin (\omega t)$, the first reset instant $t_1 \in t_R$ of $\mathcal{RCS}$ is the solution of 
	\begin{equation}
		\label{eq: t1}
		\sin \left[ \omega t_1+ \angle \mathcal{S}_{bl}(\omega)\right]=  \sum_{i=1}^{i=k}e^{p_i t_1} \sin \left( \angle \mathcal{S}_{bl}(\omega)\right).
	\end{equation}
\end{lem}
\begin{pf}
	The first reset action appears at when the base-linear error signal denoted by $e_{bl}(t)$ hits to zero. $e_{bl}(t)$ is given by \eqref{eq: ebl}, then the first solution of $e_{bl}(t_1) = 0$ is shown in \eqref{eq: t1}.
\end{pf}
Thus, 
\begin{equation}
    \sin \left[ \omega t_1+ \angle \mathcal{S}_{bl}(\omega)\right] = \sum_{i=1}^{i=k}e^{p_i t_1} \sin \left( \angle \mathcal{S}_{bl}(\omega)\right) <1,
\end{equation}
thus, 
\begin{equation}
    e_{bl}''(t_1) >0.
\end{equation}
